Making Logic Learnable With Neural Networks

While neural networks are good at learning unspecified functions from training samples, they cannot be directly implemented in hardware and are often not interpretable or formally verifiable. On the other hand, logic circuits are implementable, verifiable, and interpretable but are not able to learn from training data in a generalizable way. We propose a novel logic learning pipeline that combines the advantages of neural networks and logic circuits. Our pipeline first trains a neural network on a classification task, and then translates this, first to random forests, and then to AND-Inverter logic. We show that our pipeline maintains greater accuracy than naive translations to logic, and minimizes the logic such that it is more interpretable and has decreased hardware cost. We show the utility of our pipeline on a network that is trained on biomedical data. This approach could be applied to patient care to provide risk stratification and guide clinical decision-making.

==> sections/10_supplementary_old.tex <==
\clearpage
\section*{Appendix}
\label{appendix}

% -------------------------------------------------------
\subsection{Further Results}
\label{further_results}

The results of a broad experimental setup with multiple parameters can be found in the tables on the following pages (Table \ref{lgn_eighttotal_results}, \ref{rf_eighttotal_results}, \ref{minisat_result}, \ref{lgn_thirtytwototal_results} and \ref{rf_thirtytwototal_results}). \\

The evaluation of our methods is based on the following assumptions and limitations. We only use fully-connected neural networks which we train with Adam optimizer \cite{adam}. For the GI bleeding data set, our architecture follows the one used in a broad evaluation of machine learning models on the same data set \cite{shung2020validation}, which showed state-of-the-art results and was built out of only one hidden layer with 20 nodes. For training the real-valued neural network, we use a ReLU activation function on the input layer and on all hidden layers, while using a softmax activation function on the last layer in combination with a cross-entropy loss function. The ReLU activation function is also modeled within the logic of intermediate layers, but for the logic representation of the last layer, we use an identity mapping, followed by an argmax-function to get the final class prediction. This is done to prevent issues related to an exact approximation of the softmax function. Moreover we create only combinational circuits and leave the analysis and optimization of the timing aspects of the circuits as future work. Within the logic we make the assumtion that the multiplier entities have the double bit width as the number of total bits used in the data-, the activation- and the weight-quantization scheme (see Section \ref{quantization}). Similarly, we assume all accumulator entities (which do the summations) to have three times of the bit width as the quantization scheme. 

% -------------------------------------------------------
\subsection{Interpretable Reports}
\label{reports}

In the following, we provide an example of how reports from the logic can look like. We derive the report for a single node $l0;n0$ of the first layer from a direct translation of a neural network to arithmetic logic. It receives four input features from the data: the systolic blood pressure, the haemoglobin level, the urea level and the creatinine level. The inputs and the activations are quantized to 4 total bits and 2 fractional bits. The Boolean equations derived from the AIG of the logic module can be found in the following. Also a single logic module can potentially be simulated, using this report. The derived AIG has 134 nodes and can be visualized as shown in Figure \ref{l0n0_figure}. From this is can be quickly seen that in this example there is no dependence on the variables creatinine and urea, which means that they are internally treated as don't-cares. Similar reports can be created from any arbitrary concatenation of logic modules, allowing simulations and interpretations also of only intermediate layers or nodes or measuring variables' influences.

% \newpage
\textbf{Logic Report:} l0n0{\_}nn\\
\noindent\rule{\columnwidth}{0.4pt}

\textbf{Inputs:}\\
\noindent\rule{\columnwidth}{0.4pt}

Input 0:	systolic\\
Input 1:	haemoglobin\\
Input 2:	urea\\
Input 3:	creatinine\\

\textbf{Outputs:}\\
\noindent\rule{\columnwidth}{0.4pt}

Output:	l0n0{\_}nn{\_}out\\

\textbf{Equations:}\\
\noindent\rule{\columnwidth}{0.4pt}

n21 = systolic[0] AND systolic[1];\\
n22 = NOT systolic[0] AND NOT systolic[1];\\
n23 = NOT n21 AND NOT n22;\\
n24 = haemoglobin[0] AND n23;\\
n25 = systolic[2] AND n23;\\
n26 = NOT systolic[2] AND NOT n23;\\
n27 = NOT n25 AND NOT n26;\\
n28 = n21 AND n27;\\
n29 = NOT n21 AND NOT n27;\\
n30 = NOT n28 AND NOT n29;\\
n31 = haemoglobin[0] AND haemoglobin[1];\\
n32 = NOT haemoglobin[0] AND NOT haemoglobin[1];\\
n33 = NOT n31 AND NOT n32;\\
n34 = n30 AND n33;\\
n35 = NOT n30 AND NOT n33;\\
n36 = NOT n34 AND NOT n35;\\
n37 = n24 AND n36;\\
n38 = NOT n24 AND NOT n36;\\
n39 = NOT n37 AND NOT n38;\\
n40 = NOT systolic[0] AND systolic[1];\\
n41 = systolic[0] AND NOT systolic[1];\\
n42 = NOT n40 AND NOT n41;\\
n43 = systolic[2] AND n42;\\
n44 = NOT systolic[2] AND NOT n42;\\
n45 = NOT n43 AND NOT n44;\\
n46 = n21 AND n45;\\
n47 = NOT n21 AND NOT n45;\\
n48 = NOT n46 AND NOT n47;\\
n49 = NOT systolic[3] AND n48;\\
n50 = NOT n25 AND NOT n28;\\
n51 = systolic[3] AND NOT n48;\\
n52 = NOT n49 AND NOT n51;\\
n53 = NOT n50 AND n52;\\
n54 = NOT n49 AND NOT n53;\\
n55 = NOT n43 AND NOT n46;\\
n56 = NOT systolic[1] AND systolic[2];\\
n57 = systolic[1] AND NOT systolic[2];\\
n58 = NOT n56 AND NOT n57;\\
n59 = n40 AND n58;\\
n60 = NOT n40 AND NOT n58;\\
n61 = NOT n59 AND NOT n60;\\
n62 = NOT systolic[3] AND n61;\\
n63 = systolic[3] AND NOT n61;\\
n64 = NOT n62 AND NOT n63;\\
n65 = NOT n55 AND n64;\\
n66 = n55 AND NOT n64;\\
n67 = NOT n65 AND NOT n66;\\
n68 = n54 AND NOT n67;\\
n69 = NOT n54 AND n67;\\
n70 = NOT n68 AND NOT n69;\\
n71 = NOT haemoglobin[0] AND haemoglobin[1];\\
n72 = haemoglobin[0] AND NOT haemoglobin[1];\\
n73 = NOT n71 AND NOT n72;\\
n74 = haemoglobin[2] AND n73;\\
n75 = NOT haemoglobin[2] AND NOT n73;\\
n76 = NOT n74 AND NOT n75;\\
n77 = n31 AND n76;\\
n78 = NOT n31 AND NOT n76;\\
n79 = NOT n77 AND NOT n78;\\
n80 = NOT n74 AND NOT n77;\\
n81 = NOT haemoglobin[1] AND haemoglobin[2];\\
n82 = haemoglobin[1] AND NOT haemoglobin[2];\\
n83 = NOT n81 AND NOT n82;\\
n84 = n71 AND n83;\\
n85 = NOT n71 AND NOT n83;\\
n86 = NOT n84 AND NOT n85;\\
n87 = NOT haemoglobin[3] AND n86;\\
n88 = haemoglobin[3] AND NOT n86;\\
n89 = NOT n87 AND NOT n88;\\
n90 = NOT n80 AND n89;\\
n91 = n80 AND NOT n89;\\
n92 = NOT n90 AND NOT n91;\\
n93 = NOT n79 AND NOT n92;\\
n94 = n79 AND n92;\\
n95 = NOT n93 AND NOT n94;\\
n96 = NOT n70 AND NOT n95;\\
n97 = n50 AND NOT n52;\\
n98 = NOT n53 AND NOT n97;\\
n99 = NOT n79 AND n98;\\
n100 = NOT n34 AND NOT n37;\\
n101 = n79 AND NOT n98;\\
n102 = NOT n99 AND NOT n101;\\
n103 = NOT n100 AND n102;\\
n104 = NOT n99 AND NOT n103;\\
n105 = n70 AND n95;\\
n106 = NOT n96 AND NOT n105;\\
n107 = NOT n104 AND n106;\\
n108 = NOT n96 AND NOT n107;\\
n109 = NOT n62 AND NOT n65;\\
n110 = NOT n56 AND NOT n59;\\
n111 = NOT systolic[2] AND NOT systolic[3];\\
n112 = systolic[2] AND systolic[3];\\
n113 = NOT n111 AND NOT n112;\\
n114 = NOT n110 AND n113;\\
n115 = n110 AND NOT n113;\\
n116 = NOT n114 AND NOT n115;\\
n117 = NOT n109 AND n116;\\
n118 = n109 AND NOT n116;\\
n119 = NOT n117 AND NOT n118;\\
n120 = NOT n68 AND n119;\\
n121 = n68 AND NOT n119;\\
n122 = NOT n120 AND NOT n121;\\
n123 = NOT n87 AND NOT n90;\\
n124 = NOT n81 AND NOT n84;\\
n125 = NOT haemoglobin[2] AND NOT haemoglobin[3];\\
n126 = haemoglobin[2] AND haemoglobin[3];\\
n127 = NOT n125 AND NOT n126;\\
n128 = NOT n124 AND n127;\\
n129 = n124 AND NOT n127;\\
n130 = NOT n128 AND NOT n129;\\
n131 = NOT n123 AND n130;\\
n132 = n123 AND NOT n130;\\
n133 = NOT n131 AND NOT n132;\\
n134 = NOT n93 AND n133;\\
n135 = n93 AND NOT n133;\\
n136 = NOT n134 AND NOT n135;\\
n137 = n122 AND n136;\\
n138 = NOT n122 AND NOT n136;\\
n139 = NOT n137 AND NOT n138;\\
n140 = NOT n108 AND n139;\\
n141 = n108 AND NOT n139;\\
n142 = NOT n140 AND NOT n141;\\
n143 = n104 AND NOT n106;\\
n144 = NOT n107 AND NOT n143;\\
n145 = n100 AND NOT n102;\\
n146 = NOT n103 AND NOT n145;\\
n147 = NOT n39 AND NOT n146;\\
n148 = NOT n144 AND n147;\\
n149 = NOT n142 AND n148;\\
n150 = NOT n142 AND NOT n149;\\
l0n0{\_}nn{\_}out[0] = n39 AND n150;\\
l0n0{\_}nn{\_}out[1] = n146 AND n150;\\
l0n0{\_}nn{\_}out[2] = n144 AND n150;\\
l0n0{\_}nn{\_}out[3] = n142 AND n150;\\

% -------------------------------------------------------
\begin{figure*}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\textwidth]{imgs/l0n0_nn_aig_cut.pdf}}
\caption{Example of the AIG that is derived from a simple logic module. The visualization was exported after creating the AIG with ABC \cite{abc}.}
\label{l0n0_figure}
\end{center}
\vskip -0.2in
\end{figure*}

% -------------------------------------------------------
\begin{table*}[ht]
\caption{Results of \textbf{LogicNet} as intermediate step with the logic being quantized to \textbf{8 total bits and 6 fractional bits}. The column-wise ``winner" is marked in bold.}
\label{lgn_eighttotal_results}
\vskip 0.15in
\begin{center}
% \begin{small}
\begin{sc}
\scalebox{0.8}{
\begin{tabular}{ccccccc}
\toprule
Depth & Width & LUT-Size & AIG Nodes & AIG Levels & Logic Accuracy (\%) \\
\midrule
2 & 50 & 4 & 80,756 & 187 & 54.17 \\
2 & 100 & 4 & 71,162 & 186 & 54.00 \\
2 & 200 & 4 & \textbf{56,738} & \textbf{184} & 54.17 \\
2 & 50 & 6 & 107,190 & 188 & 54.17 \\
2 & 100 & 6 & 116,563 & 188 & 54.17 \\
2 & 200 & 6 & 176,307 & 204 & 54.17 \\
2 & 50 & 8 & 224,670 & 202 & 53.50 \\ 
2 & 100 & 8 & 217,562 & 204 & 54.33 \\ 
2 & 200 & 8 & 135,649 & 189 & 54.00 \\ 
% \midrule
3 & 50 & 4 & 239,243 & 205 & 53.50 \\ 
3 & 100 & 4 & 221,350 & 201 & 53.83 \\ 
3 & 200 & 4 & 215,211 & 206 & 54.17 \\ 
3 & 50 & 6 & 146,347 & 192 & 56.50 \\ 
3 & 100 & 6 & 249,995 & 203 & 54.00 \\ 
3 & 200 & 6 & 147,908 & 196 & 54.33 \\
3 & 50 & 8 & 149,378 & 197 & 54.17 \\
3 & 100 & 8 & 147,145 & 195 & 55.83 \\
3 & 200 & 8 & 149,399 & 196 & 54.17 \\
% \midrule
4 & 50 & 4 & 146,130 & 192 & 54.33 \\ 
4 & 100 & 4 & 146,592 & 191 & 54.17 \\ 
4 & 200 & 4 & 145,878 & 191 & 50.33 \\ 
4 & 50 & 6 & 254,011 & 209 & 54.67 \\ 
4 & 100 & 6 & 151,359 & 197 & 54.17 \\
4 & 200 & 6 & 255,886 & 205 & \textbf{58.83} \\
4 & 50 & 8 & 255,403 & 209 & 54.33 \\ 
4 & 100 & 8 & 256,910 & 212 & 56.00 \\ 
4 & 200 & 8 & 157,274 & 201 & 57.33 \\
\bottomrule
\end{tabular}
}
\end{sc}
\end{center}
\end{table*}

% -------------------------------------------------------
\begin{table*}[ht]
\caption{Results of \textbf{random forest} as intermediate step with the logic being quantized to \textbf{8 total bits and 6 fractional bits}. The column-wise ``winner" is marked in bold.}
\label{rf_eighttotal_results}
\vskip 0.15in
\begin{center}
\begin{sc}
\scalebox{0.8}{
\begin{tabular}{cccccc}
\toprule
Estimators & Max. Depth & AIG Nodes & AIG Levels & Logic Accuracy (\%) \\
% \midrule
2 & 5 & \textbf{198,378} & \textbf{227} & 54.17 \\
2 & 10 & 541,789 & 251 & 48.50 \\
2 & 15 & 472,091 & 261 & 53.50 \\
% \midrule
3 & 5 & 341,500 & 272 & 52.50 \\
3 & 10 & 737,429 & 263 & 52.00 \\
3 & 15 & 630,701 & 275 & 54.17 \\
% \midrule
4 & 5 & 266,826 & 252 & \textbf{55.00} \\
4 & 10 & 912,589 & 275 & 49.83 \\
4 & 15 & 793,930 & 287 & 48.83 \\
\bottomrule
\end{tabular}
}
\end{sc}
\end{center}
\vskip -0.1in
\end{table*}

% -------------------------------------------------------

\begin{table*}[ht]
\caption{Results of the computing times for MiniSAT \cite{een2003extensible} to find satisfying arguments for multiple settings of bloated and reduced logic - ordered by the number of AIG nodes.}
\label{minisat_result}
\vskip 0.15in
\begin{center}
% \begin{small}
\begin{sc}
\scalebox{0.8}{
\begin{tabular}{cccccc}
\toprule
Logic Translation \\($m$ total bits, $i$ fractional bits) & Settings & AIG Nodes & AIG Levels & MiniSAT time \\
\midrule
Neural Network ($32$, $16$) & - & 2,516,251 & 1,113 & 18,813.05 s (313.55 min) \\ % 01
Random Forest ($8$, $6$) & Estimators: 4; Max. Depth: 10 & 912,589 & 275 & 22,310.16 s (371.84 min) \\ % 03
LogicNet ($8$, $6$) & Depth: 4; Width: 100; LUT-Size: 8 & 256,910 & 212 & 1,264.43 s (21.07 min) \\ %AIG Opt. ! % 02
Neural Network ($8$, $4$) & - & 210,457 & 477 & 76.08 s (1.27 min) \\ % 06
Random Forest ($8$, $6$) & Estimators: 2; Max. Depth: 5 & 198,378 & 227 & 5,226.24 s (87.10 min) \\ % 05
LogicNet ($8$, $6$) & Depth: 2; Width: 200; LUT-Size: 4 & 56,738 & 184 & 4,880.07 s (81.33 min) \\ %AIG Opt. ! % 04
\bottomrule
\end{tabular}
}
\end{sc}
% \end{small}
\end{center}
% \vskip -0.1in
\end{table*}




% -------------------------------------------------------
\begin{table*}[ht]
\caption{Results of \textbf{LogicNet} as intermediate step with the logic being quantized to \textbf{32 total bits and 16 fractional bits}. The column-wise ``winner" is marked in bold.}
\label{lgn_thirtytwototal_results}
\vskip 0.15in
\begin{center}
\begin{sc}
\scalebox{0.8}{
\begin{tabular}{ccccccc}
\toprule
Depth & Width & LUT-Size & AIG Nodes & AIG Levels & Logic Accuracy (\%) \\
\midrule
2 & 50 & 4 & \textbf{207,153} & \textbf{422} & 54.17 \\
2 & 100 & 4 & 208,996 & 431 & 54.17 \\
2 & 200 & 4 & 858,284 & 493 & 56.33 \\
2 & 50 & 6 & 1,519,223 & 511 & 47.33 \\
2 & 100 & 6 & 1,437,803 & 497 & 54.50 \\
2 & 200 & 6 & 756,667 & 453 & 54.17 \\
2 & 50 & 8 & 984,625 & 454 & 51.50 \\ 
2 & 100 & 8 & 948,956 & 454 & 51.17 \\ 
2 & 200 & 8 & 1,031,077 & 450 & 53.67 \\ 
% \midrule
3 & 50 & 4 & 1,744,909 & 515 & 46.83 \\ 
3 & 100 & 4 & 1,590,823 & 514 & 54.17 \\ 
3 & 200 & 4 & 716,599 & 453 & 53.50 \\ 
3 & 50 & 6 & 238,3425 & 512 & 53.00 \\ 
3 & 100 & 6 & 2,385,562 & 517 & 53.50 \\ 
3 & 200 & 6 & 1,338,098 & 464 & 55.33 \\
3 & 50 & 8 & 1,333,842 & 462 & 46.00 \\
3 & 100 & 8 & 1,339,410 & 463 & 53.17 \\
3 & 200 & 8 & 1,345,170 & 465 & 54.33 \\
% \midrule
4 & 50 & 4 & 1,286,186 & 454 & \textbf{64.33} \\ 
4 & 100 & 4 & 1,288,754 & 461 & 56.67 \\ 
4 & 200 & 4 & 1,288,886 & 458 & 40.83 \\ 
4 & 50 & 6 & 1,343,026 & 466 & 47.50 \\ 
4 & 100 & 6 & 1,353,394 & 466 & 52.83 \\
4 & 200 & 6 & 1,360,466 & 467 & 53.50 \\
4 & 50 & 8 & 1,341,298 & 463 & 56.67 \\ 
4 & 100 & 8 & 1,349,522 & 470 & 51.33 \\ 
4 & 200 & 8 & 1,361,810 & 465 & 60.83 \\
\bottomrule
\end{tabular}
}
\end{sc}
\end{center}
\end{table*}

% -------------------------------------------------------
\begin{table*}[ht]
\caption{Results of \textbf{random forest} as intermediate step with the logic being quantized to \textbf{8 total bits and 6 fractional bits}. The column-wise ``winner" for a setting with and without AIG optimization is marked in bold.}
\label{rf_thirtytwototal_results}
\vskip 0.15in
\begin{center}
\begin{sc}
\scalebox{0.8}{
\begin{tabular}{cccccc}
\toprule
Estimators & Max. Depth & AIG Nodes & AIG Levels & Logic Accuracy (\%) \\
% \midrule
2 & 5 & \textbf{1,660,911} & \textbf{506} & 54.67 \\
2 & 10 & 2,688,533 & 530 & 52.50 \\
2 & 15 & 2,389,484 & 541 & 51.67 \\
% \midrule
3 & 5 & 1,865,767 & 519 & \textbf{55.67} \\
3 & 10 & 4,164,037 & 592 & 48.50 \\
3 & 15 & 2,934,422 & 553 & 51.67 \\
% \midrule
4 & 5 & 3,153,180 & 600 & 53.33 \\
4 & 10 & 3,458,848 & 565 & 50.00 \\
4 & 15 & 3,469,420 & 564 & 52.67 \\
\bottomrule
\end{tabular}
}
\end{sc}
\end{center}
\end{table*}

==> sections/notes.tex <==

% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to break the
% lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4 authors names on the first line, and the last on the second line, try using
% \AND instead of \And before the third author name.
% use \thanks{} for footnotes


% \author{
%   Tobias Brudermueller\\
%   Institute of Imaging and Computer Vision\\
%   RWTH Aachen University\\
%   Aachen, Germany\\
%   \texttt{tobias.brudermueller@rwth-aachen.de}\\
  
%   \And
%   Dennis L. Shung\\
%   Yale School of Medicine\\
%   Yale University\\
%   New Haven, CT, USA\\
  
%   \And
%   Loren Laine\\
%   Yale School of Medicine\\
%   Yale University\\
%   New Haven, CT, USA\\
  
%   \And
%   Adrian J. Stanley\\
%   Glasgow Royal Infirmary\\
%   Glasgow, United Kingdom
  
%   \And
%   Stig B. Laursen\\
%   Odense University Hospital\\
%   Odense, Denmark\\
  
%   \And 
%   Harry R. Dalton\\
%   Royal Cornwall Hospital\\
%   Cornwall, United Kingdom\\
  
%   \And
%   Jeffrey Ngu\\
%   Christchurch Hospital\\
%   Christchurch, New Zealand\\
  
%   \And 
%   Michael Schultz\\
%   Dunedin Hospital\\
%   Dunedin, New Zealand\\
  
%   \And
%   Johannes Stegmaier\\
%   Institute of Imaging and Computer Vision\\
%   RWTH Aachen University\\
%   Aachen, Germany\\
  
%   \And
%   Smita Krishnaswamy \\
%   Yale School of Medicine\\
%   Yale University\\
%   New Haven, CT, USA\\
%   \texttt{smita.krishnaswamy@yale.edu}
% }




% -----------------------------------------



\newcommand{\arithmeticcircuittab}{
\begin{adjustbox}{width=0.4\textwidth}
\begin{tabular}{cccccccc}
\toprule
\makecell{Reference\\Key} & \makecell{Quantization\\Scheme} &\makecell{Selection\\From} & \makecell{AIG\\Nodes} &    \makecell{AIG\\Levels} &  \makecell{Accuracy\\in \%} \\
\midrule
GIB - Small 	& (7, 3)		& Table \ref{gib_arithmetic_circuit} 	& 14,314 		&  231	& 70.36\\
GIB - Small 	& (18, 10)		& Table \ref{gib_arithmetic_circuit} 	&  123,389 	&  451 	& 83.28 \\
\midrule
VACS - Small 	& (7, 3)		& Table \ref{vacs_arithmetic_circuit} 	&  17,807 		& 183	& 35.51 \\
VACS - Small 	& (32, 16)		& Table \ref{vacs_arithmetic_circuit} 	&  338,757 	&  549 	& 63.20 \\
\midrule
GIB - Big 		& (6, 4)		& Table \ref{gib_nn_logic} 			&  38,414 		&  240	& 52.48 \\
GIB - Big 		&  (12, 8)		& Table \ref{gib_nn_logic} 			&  150,427 	&  338 	& 45.20 \\
\midrule
VACS - Big 	& (6, 4)		& Table \ref{vacs_nn_logic_big} 	&  106,572 	&  353	& 34.97 \\
VACS - Big 	&  (32, 16)		& Table \ref{vacs_nn_logic_big} 	&  2,173,117 	&  726 	& 34.97 \\
\bottomrule
\end{tabular}
\end{adjustbox}
}

\newcommand{\rftab}{
\begin{adjustbox}{width=0.4\textwidth}
\begin{tabular}{ccccccc}
\toprule
\makecell{Reference\\Key} & \makecell{Quantization\\Scheme} &\makecell{Full\\Results} & \makecell{Settings \\(Max. Tree Depth,\\Num. Estimators,\\Bitwise Training)} & \makecell{AIG\\Nodes} &    \makecell{AIG\\Levels} &  \makecell{Accuracy\\in \%} \\
\midrule
GIB - Small 	& (7, 3)		& Table \ref{rf_tb7_gib_results} 			&  (20, 3, No) 	&  50,684 			&  245		&  \textbf{83.28} \\
GIB - Small 	& (18, 10)		& Table \ref{rf_tb18_gib_results} 		&  (10, 2, No) 	&  \textbf{114,011} 	&  \textbf{357} 	&  77.65 \\
\midrule
VACS - Small 	& (7, 3)		& Table \ref{rf_tb7_vacs_results} 		&  (20, 2, No) 	&    95,176 		&  \textbf{177}	&  \textbf{49.80} \\
VACS - Small 	& (32, 16)		& Table \ref{rf_tb32_vacs_results} 		&  (10, 2, No) 	& \textbf{25,4579} 	&  \textbf{354} 	&    38.91 \\
\midrule
GIB - Big 		& (6, 4)		& Table \ref{rf_tb6_gib_big_results} 		&  (15, 3, No) 	&  425,617 		&  \textbf{213}	&  \textbf{56.29} \\
GIB - Big 		&  (12, 8)		& Table \ref{rf_tb12_gib_big_results} 	&  (20, 2, No) 	&  214,009 		&  \textbf{300} 	&  \textbf{59.27} \\
\midrule
VACS - Big 	& (6, 4)		& Table \ref{rf_tb6_vacs_big_results} 	&  (5, 3, Yes) 	&    \textbf{83,697} 	&  \textbf{146}	&  \textbf{37.69} \\
VACS - Big 	&  (32, 16)		& Table \ref{rf_tb32_vacs_big_results} 	&  (15, 4, Yes) 	& \textbf{2,097,694} 	&  \textbf{373} 	&    \textbf{39.39} \\
\bottomrule
\end{tabular}
\end{adjustbox}
}


\newcommand{\logicnettab}{
\begin{adjustbox}{width=0.4\textwidth}
\begin{tabular}{ccccccc}
\toprule
\makecell{Reference\\Key} & \makecell{Quantization\\Scheme} &\makecell{Full\\Results} & \makecell{Settings \\(Depth, Width,\\LUT Size)} & \makecell{AIG\\Nodes} &    \makecell{AIG\\Levels} &  \makecell{Accuracy\\in \%} \\
\midrule
GIB - Small 	& (7, 3)		& Table \ref{lgn_gib_small_tb7} 	&  (2, 200, 2) 	&  \textbf{2,508} 	&  \textbf{106}		&  66.56 \\
GIB - Small 	& (18, 10)		& Table \ref{lgn_gib_small_tb18} 	&  (4, 1000, 1) 	&  \textbf{25,536} 	&  \textbf{198}		&  65.56 \\
\midrule
VACS - Small 	& (7, 3)		& Table \ref{lgn_vacs_small_tb7} 	&  (2, 500, 3) 	&    \textbf{7,473} 	&  \textbf{89}		&  33.40  \\
VACS - Small 	& (32, 16)		& Table \ref{lgn_vacs_small_tb32} 	&  (3, 1000, 3) 	&   \textbf{186,572} 	&  \textbf{274}		&  33.40 \\
\midrule
GIB - Big 		& (6, 4)		& Table \ref{lgn_gib_big_tb6} 		&  (3, 50, 2) 	&  \textbf{13,501} 	&  \textbf{131}		&  \textbf{64.40} \\
GIB - Big 		&  (12, 8)		& Table \ref{lgn_gib_big_tb12} 		&  (2, 500, 2) 	&  \textbf{41,867} 	&  \textbf{165} 		&  \textbf{50.50} \\
\midrule
VACS - Big 	& (6, 4)		& Table \ref{lgn_vacs_big_tb6} 		&  (3, 200, 2) 	&   0			 	&  0				&  33.33 \\
VACS - Big 	&  (32, 16)		& Table \ref{lgn_vacs_big_tb32} 	&  (3, 500, 3) 	&  \textbf{389,577} 	&  \textbf{264}		&  33.47 \\
\bottomrule
\end{tabular}
\end{adjustbox}
}

\newcommand{\directrf}{
\begin{adjustbox}{width=0.4\textwidth}
\begin{tabular}{ccccccc}
\toprule
\makecell{Reference\\Key} & \makecell{Quantization\\Scheme} &\makecell{Full\\Results} & \makecell{Settings \\(Max. Tree Depth,\\Num. Estimators)} & \makecell{AIG\\Nodes} &    \makecell{AIG\\Levels} &  \makecell{Accuracy\\in \%} \\
\midrule
GIB - Small 	& (7, 3)		& Table \ref{rf_direct_gib_small_tb7} 		&  (5, 2) 	&  	\textbf{448} 		&  \textbf{23} 	&  	\textbf{82.12} \\
GIB - Small 	& (18, 10)		& Table \ref{rf_direct_gib_small_tb18} 	&  (5, 4) 	& 	\textbf{2,065} 	&  \textbf{94} 	&  	52.98  \\
\midrule
VACS - Small 	& (7, 3)		& Table \ref{rf_direct_vacs_small_tb7}	&  (15, 2) 	&    	\textbf{7,313} 	&  \textbf{40}		&  	\textbf{76.80} \\
VACS - Small 	& (32, 16)		& Table \ref{rf_direct_vacs_small_tb32}	&  (15, 2) 	&	\textbf{38,955} 	&  \textbf{92} 	&   	33.67 \\
\midrule
GIB - Big 		& (6, 4)		& Table \ref{rf_direct_gib_big_tb6}		&  (5, 3) 	& 	\textbf{618} 		&  \textbf{35}		&  	\textbf{80.46} \\
GIB - Big 		&  (12, 8)		& Table \ref{rf_direct_gib_big_tb12} 		&  (5, 2) 	&	\textbf{442} 		&  \textbf{36} 	&  	\textbf{59.44} \\
\midrule
VACS - Big 	& (6, 4)		& Table \ref{rf_direct_vacs_big_tb6} 		&  (20, 4) 	&	\textbf{12,601} 	&  \textbf{52}		& 	\textbf{77.07} \\
VACS - Big 	&  (32, 16)		& Table \ref{rf_direct_vacs_big_tb32} 	&  (15, 3) 	&	\textbf{40,876} 	&  \textbf{128} 	& 	34.08 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{test}
}



% \begin{figure}

% %   \qquad
%     \centering
%   \subfigure[Overview of the \textbf{selected quantization schemes} - notation: (total bits, fractional bits) and corresponding arithmetic circuits' performance. They also serve as \textbf{arithmetic circuit baselines}.]{\arithmeticcircuittab}%

%   \qquad
%   \subfigure[The results of the \textbf{top-1 random forest logic} for all data set setups and their individually selected quantization schemes.]{\rftab}
  
%   \qquad
%   \subfigure[The results of the \textbf{top-1 LogicNet logic} for all data set setups and their individually selected quantization schemes. Note that if the number of nodes or levels in the AIG is zero, this means that the LogicNet has learned nothing and its corresponding logic has a constant class prediction.]{\logicnettab}
  
%   \qquad
%   \subfigure[The results of the \textbf{top-1 direct random forest logic} for all data set setups and their individually selected quantization schemes.]{\directrf}
  
  
%   \caption{Here are some tables in a \texttt{figure} environment.}%
%   \label{fig:table}%
% \end{figure}

% \begin{table}%
%   \centering
%   \subfloat[][]{\mytab}%
%   \qquad
%   \subfloat[][]{\mytab}
%   \caption{Here are some tables in a \texttt{table} environment.}%
%   \label{tbl:table}%
% \end{table}



% \begin{table}
% \centering

% \begin{subtable}[c]{0.8\paperwidth}
% \raggedleft
% % \centering
% \logicnettab
% \subcaption{LogicNet}
% \end{subtable}

% \begin{subtable}[c]{0.8\paperwidth}
% % \centering
% \raggedright
% \rftab
% \subcaption{RandomForest}
% \end{subtable}

% \caption{Tables Test}
% \end{table}


\begin{table}
\begin{adjustbox}{width=1.0\paperwidth}
  \centering
  \subfloat[][The results of the \textbf{top-1 LogicNet logic} for all data set setups and their individually selected quantization schemes. Note that if the number of nodes or levels in the AIG is zero, this means that the LogicNet has learned nothing and its corresponding logic has a constant class prediction.]{\logicnettab}
  \label{lgn_best_logic}
  
  \qquad
  \subfloat[][The results of the \textbf{top-1 random forest logic} for all data set setups and their individually selected quantization schemes.]{\rftab}
  \label{rf_best_logic}
  
  \caption{Here are some tables in a \texttt{table} environment.}%
  \label{tbl:table}
  \end{adjustbox}
\end{table}













%---------------------------------------------------
% Combined table (excluding real-valued accuracy)
%---------------------------------------------------
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \begin{table}[]
% \centering
% \begin{adjustbox}{width=1.2\textwidth,center}
% \begin{tabular}{@{}cc|ccc|ccc|ccc|ccc@{}}
% \toprule
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Reference\\ Key\end{tabular}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Quantization \\ Scheme\end{tabular}} &
%   \multicolumn{3}{c|}{{\ul \textbf{Arithmetic Circuit}}} &
%   \multicolumn{3}{c|}{{\ul \textbf{Random Forest}}} &
%   \multicolumn{3}{c|}{{\ul \textbf{LogicNet}}} &
%   \multicolumn{3}{c}{{\ul \textbf{Direct Random Forest}}} \\
%  &
%   &
%   \begin{tabular}[c]{@{}c@{}}AIG\\ Nodes\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}AIG\\ Levels\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Accuracy\\ (in \%)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}AIG\\ Nodes\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}AIG\\ Levels\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Accuracy\\ (in \%)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}AIG\\ Nodes\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}AIG\\ Levels\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Accuracy\\ (in \%)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}AIG\\ Nodes\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}AIG\\ Levels\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Accuracy\\ (in \%)\end{tabular} \\ \midrule
% \multicolumn{1}{c|}{\multirow{2}{*}{GIB Small}}  & (7, 3)   & 1  & 2  & 3  & 4  & 5  & 6  & 7  & 8  & 9  & 10 & 11 & 12 \\
% \multicolumn{1}{c|}{}                            & (18, 10) & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 \\ \midrule
% \multicolumn{1}{c|}{\multirow{2}{*}{VACS Small}} & (7, 3)   & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 & 33 & 34 & 35 & 36 \\
% \multicolumn{1}{c|}{}                            & (32, 16) & 37 & 38 & 39 & 40 & 41 & 42 & 43 & 44 & 45 & 46 & 47 & 48 \\ \midrule
% \multicolumn{1}{c|}{\multirow{2}{*}{GIB Big}}    & (6, 4)   & 49 & 50 & 51 & 52 & 53 & 54 & 55 & 56 & 57 & 58 & 59 & 60 \\
% \multicolumn{1}{c|}{}                            & (12, 8)  & 61 & 62 & 63 & 64 & 65 & 66 & 67 & 68 & 69 & 70 & 71 & 72 \\ \midrule
% \multicolumn{1}{c|}{\multirow{2}{*}{VACS Big}}   & (6, 4)   & 73 & 74 & 75 & 76 & 77 & 78 & 79 & 80 & 81 & 82 & 83 & 84 \\
% \multicolumn{1}{c|}{}                            & (32, 16) & 85 & 86 & 87 & 88 & 89 & 90 & 91 & 92 & 93 & 94 & 95 & 96 \\ \bottomrule
% \end{tabular}%
% \end{adjustbox}
% \end{table}



%---------------------------------------------------
% Combined table (including real-valued accuracy)
%---------------------------------------------------
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[ht!]
\caption{\textcolor{red}{[TODO: Combined Table Caption. NOTE: no reference to results tables provided. Settings of winning top-1 models not mentioned.]}\\}
\label{combined_table}
\centering
\begin{adjustbox}{width=1.2\textwidth,center}
\begin{tabular}{@{}c|c|c|ccc|ccc|ccc|ccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Reference\\ Key\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Real-Valued\\ Network\\ Acc. (in \%)\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Quant. \\ Scheme\end{tabular}} &
  \multicolumn{3}{c|}{{\ul \textbf{Arithmetic Circuit}}} &
  \multicolumn{3}{c|}{{\ul \textbf{Random Forest}}} &
  \multicolumn{3}{c|}{{\ul \textbf{LogicNet}}} &
  \multicolumn{3}{c}{{\ul \textbf{Direct Random Forest}}} \\
 &
   &
   &
  \begin{tabular}[c]{@{}c@{}}AIG\\ Nodes\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}AIG\\ Levels\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Acc.\\ (in \%)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}AIG\\ Nodes\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}AIG\\ Levels\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Acc.\\ (in \%)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}AIG\\ Nodes\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}AIG\\ Levels\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Acc.\\ (in \%)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}AIG\\ Nodes\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}AIG\\ Levels\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Acc.\\ (in \%)\end{tabular} \\ \midrule
\multirow{2}{*}{GIB Small}  & \multirow{2}{*}{83.28} & (7, 3)   & 14,314  & 231  & 70.36  & 50,684  & 245  & 83.28  & 2,508  & 106  & 66.56  & 448 & 23 & 82.12 \\
                            &                    & (18, 10) & 123,389 & 451 & 83.28 & 114,011 & 357 & 77,65 & 25,536 & 198 & 65.56 & 2,065 & 94 & 52.98 \\ \midrule
\multirow{2}{*}{VACS Small} & \multirow{2}{*}{63.20} & (7, 3)   & 17,807 & 183 & 35.51 & 95,176 & 117 & 49.80 & 7,473 & 89 & 33.40 & 7,313 & 40 & 76.80 \\
                            &                    & (32, 16) & 338,757 & 549 & 63.20 & 254,579 & 354 & 38.91 & 186,572 & 274 & 33.40 & 38,955 & 92 & 33.67 \\ \midrule
\multirow{2}{*}{GIB Big}    & \multirow{2}{*}{85.93} & (6, 4)   & 38,414 & 240 & 52.48 & 425,617 & 213 & 56.29 & 13,501 & 131 & 64.40 & 618 & 35 & 80.46 \\
                            &                    & (12, 8)  & 150,427 & 338 & 45.20 & 214,009 & 300 & 59.27 & 41,867 & 165 & 50.50 & 442 & 36 & 59.44 \\ \midrule
\multirow{2}{*}{VACS Big}   & \multirow{2}{*}{75.58} & (6, 4)   & 106,572 & 353 & 34.97 & 83,697 & 146 & 37.69 & 0 & 0 & 33.33 & 12,601 & 52 & 77.07 \\
                            &                    & (32, 16) & 2,173,117 & 726 & 34.97 & 2,097,694 & 373 & 39.39 & 389,577 & 264 & 33.47 & 40,876 & 128 & 34.08 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}




% % \vspace{-3mm}
% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.7\textwidth]{imgs/Schematic01-Refined.pdf}}
% \caption{Overview of the proposed pipeline.}
% \label{overview}
% \end{center}
% \vskip -0.2in
% \end{figure}
% % \vspace{-3mm}

% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{imgs/NNTranslation.pdf}
%          \caption{Example of an arithmetic circuit.}
%          \label{fig:y equals x}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{imgs/NoneBitwiseDecisionTreeLogic.pdf}
%          \caption{Example of a random forest logic}
%          \label{fig:three sin x}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{imgs/LUT-Logic.pdf}
%          \caption{Example of a LogicNet logic.}
%          \label{fig:five over x}
%      \end{subfigure}
%         \caption{Three simple graphs}
%         \label{fig:three graphs}
% \end{figure}



% -------------------------------------------------------
\newpage
\subsection{Detailed Discussion}
\label{logic_learning_discussion}

\textcolor{red}{[TODO: probably take this section off?]}

Although our pipeline comes with a few limitations, such as currently only supporting fully-connected neural networks and classification tasks, it introduces a number of novelties, which is why the gained results are critically discussed in the following.

The fact that small neural networks as input to the pipeline perform better than large ones might be explained by the accumulator entities. A possible explanation could be that the accumulators and multipliers are prone to needing to deal with overflows and that their bit-widths should be increased. Making this an outside option and additional hyper-parameter would increase the degree of freedom and would allow for further analyses.

An additional point that was not evaluated, but might influence the results of the logic is the chosen data normalization mode. It was assumed that it only impacts the training process of real-valued neural networks and leads to different results in fitting those to the data. However, as the normalization mode also influences the value range of the data, it is something that should be further examined in the context of the quantization scheme. For example, it can be problematic if the data normalization leads to the data points being only distinguishable in nuances of the values after the decimal point. When then using a quantization scheme with too low precision for the fractions, hence, a too small number of fractional bits, the logic might not be able to generalize well just by using the "wrong" quantization scheme.

In this context it should also be mentioned that the pipeline is rather designed for using quantization schemes with lower precision than 32 total bits. Due to most computers working with 32-bit architectures, float values are internally encoded with 32 bits. Applying the quantization scheme with 32 total bits to a floating point value that is already encoded as such might just remove information that would not be necessary to be removed. Instead just the original 32-bit value could be used. Again this is something that should be taken into account and can drive further analyses. However, we used quantization schemes smaller with less than 32 total bits, because generalizing on those can significantly enhance interpretability.

The proposed method also comes along with the trade-off of how much time and resources should be spent on fitting the real-valued neural network and how much the logic in the end benefits from doing so. For now it was observed that the resources are better spent on the logic creation itself than fitting the real-valued net as well as possible. However, deeper examinations would be needed to deliver more reliable best practices

It was in general observed that the methods which relied on bitwise training performed worse than the ones using none-bitwise procedures. An explanation could be that by using only binary features, valuable information about extrema and the bit's position is lost. Also it treats each bit position equally and independently, which is incorrect. A bit-flip on the most significant bit (MSB), i.e. the first position, has a higher impact and causes a greater error than a bit-flip on the least significant bit (LSB), i.e. the last position. If this error is propagated to the next logic modules, where it is summed up with additional errors, it can in the end cause an almost random classification. This was observed across multiple experiments that used the bitwise training techniques. It can, however, be said in this context that the bitwise random forests mostly performed better than the bitwise LogicNets. A don't-care-based approach of generalization in this context outrules a factorization approach. A reason for this can be that the LogicNets rather perform naive memorization processes, which increases the risk of misclassifying a single bit (as just described).

Moving to the none-bitwise training of random forests, another problem occurs. The way the logic is implemented, it does not integrate all possible class predictions at each leaf node to combine the probabilities for each class across trees. Instead, just the single class with the highest probability is propagated. This can be problematic when some probabilities of possible classes are very close to each other, e.g. $p(class_0) = 0.48$, $p(class_1) = 0.49$ and $p(class_2) = 0.03$. Then, they might even fall into the same quantization bin for a certain quantization scheme, such that the logic can not correctly decide anymore which is the right one to propagate. Instead, maybe the $n$ classes with the highest probability could be propagated, which however leads to the need of more comparator entities. Nonetheless, making the parameter $n$ an additional hyper-parameter would still enable a trade-off of logic complexity and could maybe lead to better performance. 

Contrastingly, for the LogicNets another none-bitwise training method should be introduced, similar to the random forests. However, if the logic could benefit from this is questionable, because it is unclear if memorization in form of the full quantized data is different from bit by bit memorization. It would, however, be a more coherent way of comparison. 

Also it was not possible to find a specific pattern of hyper-parameters in general for the LogicNet and random forest approaches, which would always outrule other settings. An approach could be to apply an additional hyper-parameter search to single LogicNet and random forest modules, using the quantized activations as training data. This could exclude certain settings early on that take up a lot of computational resources, but do not lead to good results in the logic. 

Moreover, when introducing the logic implementation of the argmax function in Section \ref{rf_translation}, it was already explained that the definition of the argmax can impact the classification with logic. In particular, when it comes to data points laying close to a decision boundary. Here, the implementations just followed one definition, but its influence was not further examined, which could also drive future work.













% --------------------------------------------------------------
% \newpage
\clearpage
\subsubsection{Step 5: Direct Random Forest Evaluation}
\label{step5_detailed_results}
The tables provided in the following show the results of the logic creation with random forests trained directly on the GIB and the VACS data. Three runs per setup were performed. In each table, the results are sorted in descending manner according to the top-1 model's performance and the column-wise "winner" is marked in bold. \\

Table \ref{rf_direct_gib_small_tb7}, Table \ref{rf_direct_gib_small_tb18}, Table \ref{rf_direct_vacs_small_tb7} and Table \ref{rf_direct_vacs_small_tb32} report the results that can be compared to the logic which is derived from small neural networks. Table \ref{rf_direct_gib_big_tb6}, Table \ref{rf_direct_gib_big_tb12}, Table \ref{rf_direct_vacs_big_tb6} and Table \ref{rf_direct_vacs_big_tb32} show the results that can be compared to the logic which is derived from big neural networks.

% \clearpage
\begin{table}[ht]
%\begin{sidewaystable}
\centering
\caption{Results of the \textbf{direct random forest logic} on the \textbf{"GIB - Small"} setup for a quantization scheme of \textbf{7 total bits and 3 fractional bits}.}\label{rf_direct_gib_small_tb7}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{cccccccc}
\toprule
\makecell{Estimators} & \makecell{Max.\\Depth} & \makecell{AIG Nodes\\(Top1)} & \makecell{AIG Nodes\\(TopN)} & \makecell{AIG Levels\\(Top1)} & \makecell{AIG Levels\\(TopN)} & \makecell{Accuracy\\(Top-1)} & \makecell{Accuracy\\(Top-N)} \\
\midrule
2 &          5 &    \textbf{448} &     \textbf{448.00 (0.00)} &       \textbf{23} &      \textbf{23.00 (0.00)} &  \textbf{82.12} &    \textbf{82.12 (0.00)} \\
3 &          5 &             639 &     639.00 (0.00) &                32 &      32.00 (0.00) &           82.12 &    82.12 (0.00) \\
4 &          5 &             823 &     823.00 (0.00) &                41 &      41.00 (0.00) &           81.13 &    81.13 (0.00) \\
3 &         20 &            1,258 &  1,848.00 (511.39) &                35 &      39.00 (3.46) &           78.97 &    75.88 (2.68) \\
2 &         20 &            1,372 &    1,372.67 (2.08) &                37 &      37.00 (0.00) &           78.31 &    77.37 (0.85) \\
2 &         10 &            2,348 &   2,314.67 (29.30) &                33 &      33.00 (0.00) &           77.65 &    77.32 (0.33) \\
2 &         15 &            2,439 &   2,391.00 (45.71) &                35 &      35.33 (0.58) &           77.48 &    76.88 (0.53) \\
3 &         10 &            3,092 &   3,101.00 (21.93) &                42 &      42.00 (0.00) &           77.48 &    76.99 (0.50) \\
4 &         10 &            4,055 &   4,023.33 (27.47) &                51 &      51.00 (0.00) &           76.99 &    75.44 (1.34) \\
3 &         15 &            3,269 &    3,271.33 (2.08) &                43 &      42.33 (0.58) &           75.99 &    75.99 (0.00) \\
4 &         15 &            4,053 &   4,153.00 (87.73) &                50 &      50.67 (0.58) &           75.33 &    74.34 (0.87) \\
4 &         20 &            1,541 &   1,495.00 (60.10) &                38 &      38.00 (4.00) &            74.50 &    73.79 (0.67) \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
%\end{sidewaystable}


% --------------------------------------------------------------
\begin{table}[ht]
%\begin{sidewaystable}
\centering
\caption{Results of the \textbf{direct random forest logic} on the \textbf{"GIB - Small"} setup for a quantization scheme of \textbf{18 total bits and 10 fractional bits}.}\label{rf_direct_gib_small_tb18}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{cccccccc}
\toprule
\makecell{Estimators} & \makecell{Max.\\Depth} & \makecell{AIG Nodes\\(Top1)} & \makecell{AIG Nodes\\(TopN)} & \makecell{AIG Levels\\(Top-1)} & \makecell{AIG Levels\\(TopN)} & \makecell{Accuracy\\(Top1)} & \makecell{Accuracy\\(Top-N)} \\
\midrule
4 &          5 &            2,065 &    2,069.67 (8.08) &                94 &      94.00 (0.00) &  \textbf{52.98} &    \textbf{52.98 (0.00)} \\
4 &         20 &           16,466 &  16,479.00 (24.27) &               113 &     113.00 (0.00) &           52.81 &    52.81 (0.00) \\
2 &         15 &            8,472 &    8,470.33 (6.66) &                65 &      65.00 (0.00) &           50.33 &    50.33 (0.00) \\
4 &         10 &            8,795 &    8,793.67 (2.31) &               104 &     104.00 (0.00) &           50.33 &    50.33 (0.00) \\
\midrule
2 &         10 &            4,810 &    4,810.00 (0.00) &                58 &      58.00 (0.00) &            50.00 &    50.00 (0.00) \\
3 &         15 &           11,699 &  11,643.67 (48.43) &                88 &      88.00 (0.00) &            50.00 &    49.01 (0.86) \\
3 &         20 &           13,597 &  13,507.33 (79.39) &                90 &      90.00 (0.00) &            50.00 &    49.34 (0.57) \\
\midrule
2 &         20 &           10,090 &  10,109.33 (41.53) &                67 &      67.00 (0.00) &           49.83 &    49.72 (0.09) \\
2 &          5 &   \textbf{1,163} &    \textbf{1,163.00 (0.00)} &       \textbf{48} &      \textbf{48.00 (0.00)} &           48.34 &    48.34 (0.00) \\
3 &          5 &            1,666 &    1,666.00 (0.00) &                71 &      71.00 (0.00) &           48.34 &    48.34 (0.00) \\
3 &         10 &            6,592 &    6,592.00 (0.00) &                81 &      81.00 (0.00) &           47.85 &    47.85 (0.00) \\
4 &         15 &           14,431 &  14,421.67 (16.17) &               111 &     111.00 (0.00) &           47.68 &    47.68 (0.00) \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
%\end{sidewaystable}


% --------------------------------------------------------------
\begin{table}[ht]
%\begin{sidewaystable}
\centering
\caption{Results of the \textbf{direct random forest logic} on the \textbf{"VACS- Small"} setup for a quantization scheme of \textbf{7 total bits and 3 fractional bits}.}\label{rf_direct_vacs_small_tb7}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{cccccccc}
\toprule
\makecell{Estimators} & \makecell{Max.\\Depth} & \makecell{AIG Nodes\\(Top1)} & \makecell{AIG Nodes\\(TopN)} & \makecell{AIG Levels\\(Top1)} & \makecell{AIG Levels\\(TopN)} & \makecell{Accuracy\\(Top-1)} & \makecell{Accuracy\\(Top-N)} \\
\midrule
2 &         15 &            7,313 &     7,276.67 (79.03) &                40 &      40.00 (0.00) &   \textbf{76.80} &    \textbf{76.78 (0.04)} \\
3 &         15 &           10,411 &    10,421.33 (47.35) &                49 &      49.00 (0.00) &           76.46 &    76.21 (0.32) \\
3 &         20 &            7,038 &     7,011.33 (62.43) &                45 &      45.00 (0.00) &           76.39 &    75.80 (0.51) \\
4 &         20 &           10,038 &  10,967.00 (1626.43) &                47 &      47.67 (1.15) &           76.05 &    75.51 (0.88) \\
2 &         20 &            3,919 &      3,919.00 (0.00) &                43 &      43.00 (0.00) &           75.58 &    75.58 (0.00) \\
4 &         15 &           13,571 &    13,491.33 (73.21) &                58 &      58.00 (0.00) &           74.29 &    73.54 (0.66) \\
4 &         10 &            9,130 &      9,133.00 (4.36) &                51 &      51.00 (0.00) &           72.59 &    72.54 (0.08) \\
3 &         10 &            7,083 &      7,083.67 (1.15) &                42 &      42.00 (0.00) &           72.24 &    72.22 (0.03) \\
2 &         10 &            4,864 &      4,864.00 (0.00) &                33 &      33.00 (0.00) &           69.05 &    69.05 (0.00) \\
\midrule
4 &          5 &             908 &       908.00 (0.00) &                39 &      39.00 (0.00) &           49.73 &    49.73 (0.00) \\
2 &          5 &    \textbf{497} &       \textbf{497.00 (0.00)} &       \textbf{23} &      \textbf{23.00 (0.00)} &           49.18 &    49.18 (0.00) \\
3 &          5 &             685 &       685.00 (0.00) &                31 &      31.00 (0.00) &           48.78 &    48.78 (0.00) \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
%\end{sidewaystable}

% --------------------------------------------------------------
\begin{table}[ht]
%\begin{sidewaystable}
\centering
\caption{Results of the \textbf{direct random forest logic} on the \textbf{"VACS - Small"} setup for a quantization scheme of \textbf{32 total bits and 16 fractional bits}.}\label{rf_direct_vacs_small_tb32}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{cccccccc}
\toprule
\makecell{Estimators} & \makecell{Max.\\Depth} & \makecell{AIG Nodes\\(Top1)} & \makecell{AIG Nodes\\(TopN)} & \makecell{AIG Levels\\(Top1)} & \makecell{AIG Levels\\(TopN)} & \makecell{Accuracy\\(Top-1)} & \makecell{Accuracy\\(Top-N)} \\
\midrule
\midrule
2 &         15 &           38,955 &   38,963.33 (14.43) &                92 &      92.00 (0.00) &  \textbf{33.67} &    \textbf{33.67 (0.00)} \\
2 &          5 &   \textbf{2,152} &     \textbf{2,152.00 (0.00)} &       \textbf{74} &      \textbf{74.00 (0.00)} &            33.40 &    33.40 (0.00) \\
3 &          5 &            3,441 &     3,441.00 (0.00) &               109 &     109.00 (0.00) &            33.40 &    33.40 (0.00) \\
4 &          5 &            4,534 &     4,534.00 (0.00) &               144 &     144.00 (0.00) &            33.40 &    33.40 (0.00) \\
\midrule
2 &         10 &           20,242 &    20,242.00 (0.00) &                84 &      84.00 (0.00) &           33.33 &    33.33 (0.00) \\
3 &         10 &           30,230 &   30,222.00 (13.86) &               119 &     119.00 (0.00) &           33.33 &    33.33 (0.00) \\
3 &         15 &           52,649 &  52,430.00 (401.16) &               127 &     127.00 (0.00) &           33.33 &    33.33 (0.00) \\
3 &         20 &           57,271 &    57,271.00 (0.00) &               131 &     131.00 (0.00) &           33.33 &    33.33 (0.00) \\
4 &         10 &           36,567 &    36,567.00 (0.00) &               154 &     154.00 (0.00) &           33.33 &    33.33 (0.00) \\
4 &         15 &           61,337 &  61,214.33 (212.46) &               162 &     162.00 (0.00) &           33.33 &    33.33 (0.00) \\
4 &         20 &           66,363 &    66,359.00 (6.93) &               166 &     166.00 (0.00) &           33.33 &    33.33 (0.00) \\
2 &         20 &           46,063 &    46,063.00 (0.00) &                96 &      96.00 (0.00) &            33.20 &    33.20 (0.00) \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
%\end{sidewaystable}

% --------------------------------------------------------------
\begin{table}[ht]
%\begin{sidewaystable}
\centering
\caption{Results of the \textbf{direct random forest logic} on the \textbf{"GIB -Big"} setup for a quantization scheme of \textbf{6 total bits and 4 fractional bits}.}\label{rf_direct_gib_big_tb6}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{cccccccc}
\toprule
\makecell{Estimators} & \makecell{Max.\\Depth} & \makecell{AIG Nodes\\(Top1)} & \makecell{AIG Nodes\\(TopN)} & \makecell{AIG Levels\\(Top1)} & \makecell{AIG Levels\\(TopN)} & \makecell{Accuracy\\(Top-1)} & \makecell{Accuracy\\(Top-N)} \\
\midrule
3 &          5 &             618 &    618.00 (0.00) &                35 &      35.00 (0.00) &  \textbf{80.46} &    \textbf{80.46 (0.00)} \\
4 &          5 &             808 &    808.00 (0.00) &                46 &      46.00 (0.00) &            80.30 &    80.30 (0.00) \\
2 &          5 &    \textbf{425} &    \textbf{425.00 (0.00)} &       \textbf{24} &      \textbf{24.00 (0.00)} &           80.13 &    80.13 (0.00) \\
2 &         10 &            2,418 &  2,401.67 (28.29) &                34 &      34.00 (0.00) &            79.80 &    78.92 (1.53) \\
3 &         10 &            3,283 &   3,276.33 (5.77) &                45 &      45.00 (0.00) &           77.81 &    77.59 (0.19) \\
3 &         20 &            1,211 &   1,211.00 (0.00) &                36 &      36.00 (0.00) &           76.82 &    76.82 (0.00) \\
4 &         15 &            4,030 &  4,042.00 (69.78) &                57 &      58.00 (1.00) &           75.99 &    73.01 (2.76) \\
2 &         15 &            2,340 &  2,326.00 (24.25) &                37 &      37.00 (0.00) &            75.50 &    74.78 (1.25) \\
3 &         15 &            3,194 &  3,161.33 (28.29) &                48 &      47.33 (0.58) &            75.50 &    74.29 (1.05) \\
4 &         10 &            4,206 &  4,209.00 (15.72) &                56 &      56.00 (0.00) &           74.17 &    73.79 (0.53) \\
2 &         20 &            2,157 &   2,156.67 (5.51) &                44 &      44.00 (0.00) &           73.84 &    73.23 (0.78) \\
4 &         20 &            1,364 &  1,384.00 (17.32) &                36 &      39.33 (2.89) &           72.19 &    71.08 (0.96) \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
%\end{sidewaystable}

% --------------------------------------------------------------
\begin{table}[ht]
%\begin{sidewaystable}
\centering
\caption{Results of the \textbf{direct random forest logic} on the \textbf{"GIB - Big"} setup for a quantization scheme of \textbf{12 total bits and 8 fractional bits}.}\label{rf_direct_gib_big_tb12}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{cccccccc}
\toprule
\makecell{Estimators} & \makecell{Max.\\Depth} & \makecell{AIG Nodes\\(Top1)} & \makecell{AIG Nodes\\(TopN)} & \makecell{AIG Levels\\(Top1)} & \makecell{AIG Levels\\(TopN)} & \makecell{Accuracy\\(Top-1)} & \makecell{Accuracy\\(Top-N)} \\
\midrule
2 &          5 &    \textbf{442} &    \textbf{442.00 (0.00)} &       \textbf{36} &      \textbf{36.00 (0.00)} &  \textbf{59.44} &    \textbf{59.44 (0.00)} \\
3 &         20 &            8,186 &  8,258.67 (62.93) &                77 &      76.33 (0.58) &           57.62 &    57.07 (0.48) \\
3 &          5 &             791 &    791.00 (0.00) &                55 &      55.00 (0.00) &           55.13 &    55.13 (0.00) \\
3 &         15 &            7,319 &   7,319.00 (0.00) &                74 &      74.00 (0.00) &           52.65 &    52.65 (0.00) \\
4 &          5 &            1,019 &   1,019.00 (0.00) &                74 &      74.00 (0.00) &           51.99 &    51.99 (0.00) \\
4 &         15 &            9,573 &   9,573.33 (0.58) &                93 &      93.00 (0.00) &           50.99 &    50.99 (0.00) \\
2 &         15 &            5,224 &   5,224.00 (0.00) &                55 &      55.00 (0.00) &            50.50 &    50.50 (0.00) \\
\midrule
2 &         10 &            2,582 &   2,582.00 (0.00) &                47 &      47.00 (0.00) &           47.52 &    47.52 (0.00) \\
3 &         10 &            3,843 &   3,840.00 (5.20) &                66 &      66.00 (0.00) &           47.35 &    47.35 (0.00) \\
4 &         20 &           10,051 &  9,961.00 (95.97) &                97 &      96.33 (1.15) &           47.02 &    47.02 (0.00) \\
4 &         10 &            5,077 &   5,077.00 (0.00) &                85 &      85.00 (0.00) &           44.37 &    44.37 (0.00) \\
2 &         20 &            6,514 &   6,512.33 (2.89) &                60 &      60.00 (0.00) &           43.87 &    43.87 (0.00) \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
%\end{sidewaystable}


% --------------------------------------------------------------
\begin{table}[ht]
%\begin{sidewaystable}
\centering
\caption{Results of the \textbf{direct random forest logic} on the \textbf{"VACS - Big"} setup for a quantization scheme of \textbf{6 total bits and 4 fractional bits}.}\label{rf_direct_vacs_big_tb6}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{cccccccc}
\toprule
\makecell{Estimators} & \makecell{Max.\\Depth} & \makecell{AIG Nodes\\(Top1)} & \makecell{AIG Nodes\\(TopN)} & \makecell{AIG Levels\\(Top1)} & \makecell{AIG Levels\\(TopN)} & \makecell{Accuracy\\(Top-1)} & \makecell{Accuracy\\(Top-N)} \\
\midrule
4 &         20 &           12,601 &  12,478.00 (122.50) &                52 &      50.67 (1.53) &  \textbf{77.07} &    76.35 (0.62) \\
4 &         15 &           13,930 &   13,913.00 (34.77) &                64 &      64.00 (0.00) &           76.94 &   \textbf{76.94 (0.00)} \\
3 &         20 &            9,622 &    9,582.33 (43.39) &                45 &      45.00 (0.00) &            76.80 &    76.44 (0.63) \\
2 &         15 &            7,518 &     7,515.00 (2.65) &                42 &      42.00 (0.00) &           76.26 &    76.21 (0.04) \\
2 &         20 &            6,700 &    6,747.67 (41.28) &                43 &      43.00 (0.00) &           76.12 &    75.81 (0.27) \\
4 &         10 &            9,397 &    9,397.67 (46.00) &                56 &      56.00 (0.00) &           74.42 &    73.44 (1.11) \\
3 &         15 &           10,692 &   10,732.67 (35.23) &                53 &      53.00 (0.00) &           73.88 &    73.83 (0.04) \\
3 &         10 &            7,124 &    7,118.00 (10.39) &                45 &      45.00 (0.00) &           72.72 &    72.68 (0.08) \\
2 &         10 &            4,841 &     4,841.00 (0.00) &                34 &      34.00 (0.00) &           68.57 &    68.57 (0.00) \\
\midrule
3 &          5 &             679 &      679.00 (0.00) &                34 &      34.00 (0.00) &           49.66 &    49.66 (0.00) \\
4 &          5 &             914 &      914.00 (0.00) &                45 &      45.00 (0.00) &           49.59 &    49.59 (0.00) \\
2 &          5 &    \textbf{478} &      \textbf{478.00 (0.00)} &       \textbf{23} &      \textbf{23.00 (0.00)} &           47.41 &    47.41 (0.00) \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
%\end{sidewaystable}

% --------------------------------------------------------------
\begin{table}[ht]
%\begin{sidewaystable}
\centering
\caption{Results of the \textbf{direct random forest logic} on the \textbf{"VACS - Big"} setup for a quantization scheme of \textbf{32 total bits and 16 fractional bits}.}\label{rf_direct_vacs_big_tb32}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{cccccccc}
\toprule
\makecell{Estimators} & \makecell{Max.\\Depth} & \makecell{AIG Nodes\\(Top1)} & \makecell{AIG Nodes\\(TopN)} & \makecell{AIG Levels\\(Top1)} & \makecell{AIG Levels\\(TopN)} & \makecell{Accuracy\\(Top-1)} & \makecell{Accuracy\\(Top-N)} \\
\midrule
3 &         15 &           40,876 &   40,882.67 (11.55) &               128 &     128.00 (0.00) &  \textbf{34.08} &    \textbf{34.08 (0.00)} \\
3 &          5 &            3,022 &     3,022.00 (0.00) &               109 &     109.00 (0.00) &           34.01 &    34.01 (0.00) \\
4 &         10 &           26,695 &   26,703.33 (14.43) &               154 &     154.00 (0.00) &           33.81 &    33.81 (0.00) \\
2 &         10 &           16,707 &    16,707.33 (1.53) &                84 &      84.00 (0.00) &           33.74 &    33.60 (0.24) \\
4 &         20 &           56,801 &  56,667.00 (119.38) &               169 &     169.00 (0.00) &           33.74 &    33.74 (0.00) \\
2 &         20 &           39,439 &  39,516.67 (134.52) &                99 &      99.00 (0.00) &           33.54 &    33.40 (0.24) \\
3 &         20 &           49,445 &   49,447.67 (20.13) &               134 &     134.00 (0.00) &            33.40 &    33.40 (0.00) \\
\midrule
2 &         15 &           34,738 &  34,606.67 (134.61) &                93 &      93.00 (0.00) &           33.33 &    33.08 (0.43) \\
3 &         10 &           21,275 &    21,274.00 (1.00) &               119 &     119.00 (0.00) &           33.33 &    33.33 (0.00) \\
\midrule
4 &         15 &           50,535 &  5,0490.00 (219.00) &               163 &     163.00 (0.00) &           32.86 &    32.86 (0.00) \\
2 &          5 &   \textbf{2,119} &     \textbf{2,119.00 (0.00)} &       \textbf{74} &      \textbf{74.00 (0.00)} &           32.52 &    32.52 (0.00) \\
4 &          5 &            4,063 &     4,063.00 (0.00) &               144 &     144.00 (0.00) &           32.18 &    32.18 (0.00) \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}




% -------------------------------------------------------
% \subsection{Direct Random Forest}
% \label{direct_rf_translation}

% For many data science domains in the biomedical context, random forests have proven to be a good tool of choice and easier to fit the data than neural networks. Moreover, they are equipped with higher interpretability than neural networks, due to the nature of the derived decision rules being readable. It is, therefore, of interest to evaluate if training random forests on the data directly and then translating them to logic can also lead to generalization. Thus, this procedure is provided as an additional method, next to the previously described framework (Section \ref{framework}) of training neural networks, deriving intermediate representations and multiple translations to logic. Throughout the rest of the thesis it is referred to this procedure as \emph{direct random forest}. \\ 

% Within that, the identical translation to logic is used as previously described for the none-bitwise training of random forests. The training is done on the data directly instead of using neural network activations. But beforehand the quantization scheme (Section \ref{quantization}) is applied directly to the data, using the unsigned integer representations. The class labels of the data are used as "solutions" to the supervised classification task.



% -------------------------------------------------------------
\subsubsection{Real-Valued Neural Networks}
\label{step1_detailed_results}
The tables provided in the following show the results in terms of the accuracy measure for training real-valued neural networks on the GIB data set and the VACS data set. For each of the data sets different architectures, optimizers and normalization modes were used and three runs per configuration were executed. In each table, the results are sorted in descending manner according to the top-1 model's performance and the column-wise "winner" is marked in bold.

\textcolor{red}{[TODO: provide more details about the search for appropriate architectures or remove it!}

Note that abbreviations are used to encode the data normalization mode: 
\begin{enumerate}
\item Z-Score Normalization
\item Min-Max-Scaling
\item Max-Abs-Scaling
\item Robust-Scaling
\item Power-Transforming
\item Quantile-Transforming
\item Independent Normalization
\end{enumerate}


% -------------------------------------------------------------
\begin{center}
 \begin{small}
\begin{longtable}{cccccc}
\caption{\small The real-valued neural network models after training different configurations on the \textbf{GIB data set}. \textcolor{red}{TODO: fill in the additional runs of the small networks!}}\label{gib_nn_baseline}\\
\toprule
\makecell{Row\\Index} & \makecell{Hidden Layer\\Nodes} &   \makecell{Optimizer} & \makecell{Normalization\\Mode} & \makecell{Accuracy: Top-1\\in \%} & \makecell{Accuracy: Top-3\\Mean (Stdv.) in \%} \\
\midrule
\endhead
\midrule
\multicolumn{6}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
0   &            12 - 10 &        Adam &                  4 &  \textbf{85.93} &    83.22 (2.36) \\
1   &          8 - 6 - 3 &       AdamW &                  6 &           85.76 &    83.17 (2.32) \\
2   &       15 - 12 - 10 &         SGD &                  5 &           85.76 &    82.95 (2.82) \\
3   &          8 - 6 - 3 &       RAdam &                  3 &           85.43 &    82.56 (2.51) \\
4   &          8 - 6 - 3 &       RAdam &                  6 &           84.77 &    81.29 (3.15) \\
5   &              6 - 4 &        Adam &                  5 &           84.77 &    \textbf{83.66 (1.01)} \\
6   &              6 - 4 &       AdamW &                  4 &            84.6 &    82.39 (1.98) \\
7  &            12 - 10 &       RAdam &                  3 &            84.6 &    81.35 (2.83) \\
8  &            12 - 10 &        Adam &                  6 &           84.44 &    83.17 (1.66) \\
9  &            27 - 20 &        Adam &                  6 &           84.44 &    82.56 (1.91) \\
10  &       15 - 12 - 10 &         SGD &                  1 &           84.44 &    81.62 (2.45) \\
11  &       15 - 12 - 10 &       AdamW &                  5 &           84.27 &    82.17 (1.85) \\
12  &            12 - 10 &       RAdam &                  6 &           84.27 &    83.00 (1.10) \\
13  &            27 - 20 &       AdamW &                  4 &           84.11 &    82.18 (2.08) \\
14  &            12 - 10 &        Adam &                  2 &           84.11 &    83.39 (0.67) \\
15  &            12 - 10 &       RAdam &                  7 &           84.11 &    82.95 (1.47) \\
16  &          8 - 6 - 3 &       AdamW &                  7 &           83.94 &    82.78 (1.04) \\
17  &            27 - 20 &       AdamW &                  5 &           83.94 &    82.34 (1.41) \\
18  &              6 - 4 &         SGD &                  1 &           83.94 &    82.50 (1.82) \\
19  &       15 - 12 - 10 &       RAdam &                  4 &           83.94 &    82.01 (1.91) \\
20  &       15 - 12 - 10 &        Adam &                  6 &           83.77 &    82.34 (1.59) \\
21  &       15 - 12 - 10 &       AdamW &                  3 &           83.77 &    82.23 (1.49) \\
22  &            27 - 20 &        Adam &                  4 &           83.77 &    82.34 (1.59) \\
23  &            12 - 10 &       AdamW &                  5 &           83.77 &    81.46 (3.59) \\
24  &              6 - 4 &       RAdam &                  5 &           83.77 &    81.84 (2.41) \\
25  &          8 - 6 - 3 &       RAdam &                  4 &           83.77 &    83.17 (0.58) \\
26  &       15 - 12 - 10 &         SGD &                  4 &           83.77 &    81.56 (2.64) \\
27  &            27 - 20 &       RAdam &                  7 &           83.61 &    82.01 (2.22) \\
28  &              6 - 4 &       RAdam &                  2 &           83.61 &    82.56 (1.28) \\
29  &            27 - 20 &       RAdam &                  6 &           83.61 &    81.84 (1.82) \\
30  &              6 - 4 &       AdamW &                  2 &           83.61 &    82.28 (1.63) \\
31  &              6 - 4 &       RAdam &                  6 &           83.61 &    81.73 (1.70) \\
32  &            12 - 10 &       RAdam &                  5 &           83.61 &    82.78 (0.83) \\
33  &            12 - 10 &       AdamW &                  6 &           83.61 &    82.45 (1.04) \\
34  &          8 - 6 - 3 &       RAdam &                  1 &           83.61 &    81.79 (2.11) \\
35  &          8 - 6 - 3 &       RAdam &                  7 &           83.61 &    81.29 (2.71) \\
36  &          8 - 6 - 3 &        Adam &                  4 &           83.44 &    82.39 (0.99) \\
37  &          8 - 6 - 3 &       RAdam &                  2 &           83.44 &    83.28 (0.17) \\
38  &            12 - 10 &        Adam &                  5 &           83.44 &    82.28 (1.73) \\
39  &       15 - 12 - 10 &        Adam &                  4 &           83.44 &    81.68 (1.56) \\
40  &       15 - 12 - 10 &       RAdam &                  1 &           83.44 &    82.28 (1.01) \\
41  &       15 - 12 - 10 &       RAdam &                  6 &           83.44 &    82.23 (1.45) \\
42  &            27 - 20 &       AdamW &                  7 &           83.44 &    81.84 (1.50) \\
43  &          8 - 6 - 3 &       AdamW &                  5 &           83.44 &    82.12 (2.01) \\
44  &            12 - 10 &         SGD &                  1 &           83.44 &    82.62 (1.29) \\
45  &            12 - 10 &         SGD &                  5 &           83.44 &    81.84 (2.22) \\
46  &       15 - 12 - 10 &       AdamW &                  1 &           83.44 &    81.12 (2.24) \\
47  &          8 - 6 - 3 &       AdamW &                  2 &           83.28 &    82.17 (1.27) \\
48  &          8 - 6 - 3 &       AdamW &                  1 &           83.28 &    82.62 (0.76) \\
49  &              6 - 4 &        Adam &                  7 &           83.28 &    82.01 (1.25) \\
50  &       15 - 12 - 10 &       AdamW &                  7 &           83.28 &    81.57 (1.93) \\
51  &            27 - 20 &       AdamW &                  6 &           83.28 &    81.84 (1.29) \\
52  &              6 - 4 &        Adam &                  2 &           83.28 &    82.07 (1.82) \\
53  &            12 - 10 &       RAdam &                  2 &           83.28 &    81.18 (2.00) \\
54  &          8 - 6 - 3 &        Adam &                  3 &           83.11 &    82.34 (1.06) \\
55  &              6 - 4 &         SGD &                  4 &           83.11 &    81.57 (1.43) \\
56  &       15 - 12 - 10 &       RAdam &                  7 &           83.11 &    81.79 (1.25) \\
57  &       15 - 12 - 10 &       AdamW &                  6 &           83.11 &    82.17 (0.99) \\
58  &            27 - 20 &       AdamW &                  2 &           82.95 &    81.62 (1.88) \\
59  &            27 - 20 &        Adam &                  3 &           82.95 &    80.13 (2.61) \\
60  &              6 - 4 &       AdamW &                  6 &           82.95 &    81.79 (1.25) \\
61  &            12 - 10 &       AdamW &                  2 &           82.95 &    81.62 (1.20) \\
62  &            12 - 10 &       AdamW &                  4 &           82.95 &    82.01 (1.35) \\
63  &          8 - 6 - 3 &        Adam &                  6 &           82.78 &    82.17 (0.53) \\
64  &            27 - 20 &       AdamW &                  1 &           82.78 &    81.84 (1.22) \\
65  &          8 - 6 - 3 &         SGD &                  6 &           82.78 &    81.90 (0.91) \\
66  &            27 - 20 &       AdamW &                  3 &           82.78 &    81.35 (1.41) \\
67  &       15 - 12 - 10 &        Adam &                  5 &           82.78 &    82.45 (0.44) \\
68  &          8 - 6 - 3 &        Adam &                  1 &           82.78 &    81.18 (2.49) \\
69  &              6 - 4 &        Adam &                  6 &           82.78 &    80.96 (1.58) \\
70  &            27 - 20 &       RAdam &                  3 &           82.78 &    79.97 (2.47) \\
71  &              6 - 4 &       RAdam &                  4 &           82.78 &    82.51 (0.34) \\
72  &            27 - 20 &         SGD &                  6 &           82.78 &    81.79 (1.58) \\
73  &              6 - 4 &        Adam &                  1 &           82.62 &    82.34 (0.35) \\
74  &              6 - 4 &       AdamW &                  1 &           82.62 &    81.85 (1.34) \\
75  &            12 - 10 &        Adam &                  3 &           82.62 &    81.24 (1.41) \\
76  &            27 - 20 &         SGD &                  1 &           82.62 &    80.46 (2.16) \\
77  &            27 - 20 &        Adam &                  5 &           82.62 &    81.07 (2.13) \\
78  &       15 - 12 - 10 &        Adam &                  2 &           82.62 &    81.73 (0.92) \\
79  &            12 - 10 &        Adam &                  7 &           82.62 &    82.40 (0.39) \\
80 &              6 - 4 &       RAdam &                  1 &           82.62 &    82.12 (0.72) \\
81 &              6 - 4 &       AdamW &                  3 &           82.62 &    82.07 (0.82) \\
82 &            27 - 20 &        Adam &                  2 &           82.45 &    81.35 (0.97) \\
83 &       15 - 12 - 10 &        Adam &                  1 &           82.45 &    81.95 (0.60) \\
84 &              6 - 4 &       AdamW &                  5 &           82.45 &    81.24 (1.05) \\
85 &          8 - 6 - 3 &         SGD &                  5 &           82.45 &    81.95 (0.72) \\
86 &          8 - 6 - 3 &        Adam &                  2 &           82.45 &    81.95 (0.86) \\
87 &            27 - 20 &       RAdam &                  4 &           82.45 &    81.90 (0.48) \\
88 &            12 - 10 &       RAdam &                  4 &           82.45 &    81.18 (1.66) \\
89 &          8 - 6 - 3 &       AdamW &                  4 &           82.45 &    80.90 (1.49) \\
90 &       15 - 12 - 10 &       AdamW &                  2 &           82.45 &    81.18 (1.33) \\
91 &            27 - 20 &        Adam &                  7 &           82.28 &    81.07 (1.24) \\
92 &          8 - 6 - 3 &       AdamW &                  3 &           82.28 &    82.01 (0.34) \\
93 &       15 - 12 - 10 &       AdamW &                  4 &           82.28 &    82.06 (0.25) \\
94 &            12 - 10 &         SGD &                  6 &           82.28 &    80.57 (1.50) \\
95 &       15 - 12 - 10 &       RAdam &                  2 &           82.28 &    81.12 (1.60) \\
96 &              6 - 4 &        Adam &                  4 &           82.28 &    81.23 (1.08) \\
97 &            12 - 10 &       AdamW &                  3 &           82.28 &    81.35 (0.99) \\
98 &            12 - 10 &       AdamW &                  7 &           82.28 &    81.68 (0.67) \\
99 &          8 - 6 - 3 &        Adam &                  7 &           82.28 &    81.79 (0.50) \\
100 &          8 - 6 - 3 &         SGD &                  4 &           82.28 &    78.14 (3.91) \\
101 &              6 - 4 &         SGD &                  6 &           82.28 &    80.79 (1.68) \\
102 &            12 - 10 &        Adam &                  1 &           82.12 &    82.06 (0.10) \\
103 &            27 - 20 &        Adam &                  1 &           82.12 &    80.96 (1.01) \\
104 &              6 - 4 &       RAdam &                  3 &           82.12 &    81.73 (0.67) \\
105 &            27 - 20 &       RAdam &                  5 &           82.12 &    81.84 (0.25) \\
106 &       15 - 12 - 10 &         SGD &                  6 &           81.95 &    81.68 (0.25) \\
107 &              6 - 4 &         SGD &                  5 &           81.95 &    80.24 (1.50) \\
108 &          8 - 6 - 3 &       RAdam &                  5 &           81.95 &    81.40 (0.82) \\
109 &       15 - 12 - 10 &       RAdam &                  3 &           81.95 &    80.96 (1.19) \\
110 &              6 - 4 &        Adam &                  3 &           81.95 &    80.90 (1.41) \\
111 &          8 - 6 - 3 &        Adam &                  5 &           81.95 &    81.35 (0.67) \\
112 &            12 - 10 &       AdamW &                  1 &           81.79 &    81.40 (0.54) \\
113 &            12 - 10 &         SGD &                  4 &           81.46 &    79.91 (2.53) \\
114 &       15 - 12 - 10 &        Adam &                  3 &           81.46 &    81.24 (0.25) \\
115 &            27 - 20 &         SGD &                  5 &           81.46 &    80.63 (0.76) \\
116 &       15 - 12 - 10 &        Adam &                  7 &           81.46 &    80.90 (0.51) \\
117 &              6 - 4 &       AdamW &                  7 &           81.29 &    80.63 (0.60) \\
118 &              6 - 4 &       RAdam &                  7 &           81.13 &    79.91 (1.07) \\
119 &       15 - 12 - 10 &       RAdam &                  5 &           81.13 &    80.52 (1.06) \\
120 &            27 - 20 &         SGD &                  4 &           80.96 &    80.08 (0.76) \\
121 &          8 - 6 - 3 &         SGD &                  1 &           80.96 &    79.58 (1.22) \\
122 &            27 - 20 &       RAdam &                  1 &           80.79 &    80.57 (0.19) \\
123 &            27 - 20 &       RAdam &                  2 &           80.63 &    79.86 (0.75) \\
124 &            12 - 10 &       RAdam &                  1 &           80.46 &    79.91 (0.82) \\
125 &       15 - 12 - 10 &         SGD &                  2 &           78.97 &    75.05 (4.57) \\
126 &            27 - 20 &         SGD &                  3 &           78.48 &    76.88 (2.22) \\
127 &          8 - 6 - 3 &         SGD &                  7 &           77.98 &   64.29 (14.00) \\
128 &       15 - 12 - 10 &         SGD &                  3 &           77.98 &    72.85 (8.32) \\
129 &              6 - 4 &         SGD &                  2 &           77.98 &    71.85 (6.78) \\
130 &            27 - 20 &         SGD &                  7 &           77.48 &    74.72 (2.53) \\
131 &            27 - 20 &         SGD &                  2 &           77.32 &    77.10 (0.19) \\
132 &          8 - 6 - 3 &         SGD &                  3 &           76.99 &   61.42 (13.96) \\
133 &              6 - 4 &         SGD &                  3 &           76.32 &    69.31 (8.56) \\
134 &            12 - 10 &         SGD &                  7 &           75.99 &   66.39 (14.26) \\
135 &       15 - 12 - 10 &         SGD &                  7 &           75.66 &    67.82 (7.87) \\
136 &          8 - 6 - 3 &         SGD &                  2 &            75.5 &   63.91 (12.91) \\
137 &            12 - 10 &         SGD &                  2 &           75.33 &    75.06 (0.34) \\
138 &            12 - 10 &         SGD &                  3 &            75.0 &    73.56 (2.07) \\
139 &              6 - 4 &         SGD &                  7 &           74.67 &   66.34 (14.15) \\
\end{longtable}
\end{small}
\end{center}


% -------------------------------------------------------------
% \newpage
\begin{center}
\begin{small}
\begin{longtable}{cccccc}
\caption{\small The real-valued neural network models after training different configurations on the \textbf{VACS data set}. \textcolor{red}{TODO: fill in the additional runs of the small networks!}}\label{vacs_nn_baseline}\\
\toprule
\makecell{Row\\Index} & \makecell{Hidden Layer\\Nodes} &   \makecell{Optimizer} & \makecell{Normalization\\Mode} & \makecell{Accuracy: Top-1\\in \%} & \makecell{Accuracy: Top-3\\Mean (Stdv.) in \%} \\
\midrule
\endhead
\midrule
\multicolumn{6}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
0   &            40 - 20 &     RAdam &                  4 &  \textbf{75.58} &    73.11 (2.49) \\
1   &            40 - 20 &     AdamW &                  1 &           75.17 &    72.36 (2.53) \\
2   &            40 - 20 &     AdamW &                  4 &           75.03 &    \textbf{74.49 (0.88)} \\
3   &            40 - 20 &      Adam &                  4 &           74.56 &    71.65 (2.61) \\
4   &            40 - 20 &     AdamW &                  5 &           73.74 &    71.77 (2.04) \\
5   &            40 - 20 &      Adam &                  1 &           73.67 &    73.22 (0.79) \\
6   &            40 - 20 &     RAdam &                  5 &           73.27 &    72.70 (0.49) \\
7   &            40 - 20 &     RAdam &                  1 &           73.27 &    71.59 (1.46) \\
8   &       40 - 30 - 20 &       SGD &                  1 &           73.13 &    71.50 (2.37) \\
9   &            40 - 20 &      Adam &                  5 &           73.06 &    71.70 (1.44) \\
10  &            40 - 20 &     RAdam &                  6 &           72.86 &    69.96 (2.55) \\
11  &       40 - 30 - 20 &       SGD &                  5 &           72.11 &    70.89 (1.07) \\
12  &       40 - 30 - 20 &     RAdam &                  6 &           70.34 &    68.39 (1.77) \\
13  &       30 - 20 - 17 &      Adam &                  5 &            70.20 &    65.33 (4.90) \\
14  &       30 - 20 - 17 &       SGD &                  1 &            70.20 &    68.91 (1.14) \\
15  &       30 - 20 - 17 &     RAdam &                  1 &            70.00 &    67.53 (3.13) \\
16  &       40 - 30 - 20 &     AdamW &                  1 &           69.39 &    67.24 (1.87) \\
17  &       30 - 20 - 17 &      Adam &                  4 &           69.32 &    67.01 (2.76) \\
18  &            40 - 20 &     AdamW &                  6 &           69.25 &    66.05 (3.86) \\
19  &       40 - 30 - 20 &      Adam &                  1 &           69.25 &    67.71 (1.38) \\
20  &       40 - 30 - 20 &       SGD &                  4 &           69.18 &    68.34 (1.45) \\
21  &       30 - 20 - 17 &     AdamW &                  1 &           69.18 &    68.41 (1.28) \\
22  &       30 - 20 - 17 &      Adam &                  1 &           68.78 &    66.78 (2.57) \\
23  &       40 - 30 - 20 &      Adam &                  4 &           68.64 &    65.99 (2.34) \\
24  &       30 - 20 - 17 &       SGD &                  4 &           67.96 &    66.94 (1.18) \\
25  &       30 - 20 - 17 &       SGD &                  5 &           67.76 &    65.40 (2.06) \\
26  &       40 - 30 - 20 &     RAdam &                  1 &           67.55 &   59.48 (12.48) \\
27  &       40 - 30 - 20 &     AdamW &                  4 &           67.41 &    64.49 (4.00) \\
28  &       30 - 20 - 17 &     RAdam &                  4 &           67.41 &    65.03 (3.23) \\
29  &       30 - 20 - 17 &     RAdam &                  6 &           67.14 &    65.83 (1.33) \\
30  &       30 - 20 - 17 &     RAdam &                  5 &           66.39 &    65.40 (1.61) \\
31  &       40 - 30 - 20 &     AdamW &                  5 &           66.33 &    63.45 (2.68) \\
32  &            40 - 20 &      Adam &                  6 &           65.92 &    63.56 (2.38) \\
33  &       40 - 30 - 20 &      Adam &                  6 &           65.71 &    64.67 (0.91) \\
34  &       40 - 30 - 20 &      Adam &                  5 &           65.51 &    63.63 (2.06) \\
35  &       30 - 20 - 17 &      Adam &                  6 &           65.03 &    63.02 (2.61) \\
36  &            40 - 20 &       SGD &                  5 &           64.76 &    63.47 (1.12) \\
37  &       40 - 30 - 20 &     AdamW &                  6 &           64.63 &    64.06 (0.81) \\
38  &            40 - 20 &     RAdam &                  2 &           64.42 &    63.54 (0.77) \\
39  &        10 - 8 - 17 &     RAdam &                  1 &           64.35 &    63.31 (1.26) \\
40  &         10 - 7 - 4 &      Adam &                  1 &           64.08 &    61.79 (2.04) \\
41  &            40 - 20 &       SGD &                  1 &           64.01 &    63.31 (0.65) \\
42  &       40 - 30 - 20 &     RAdam &                  4 &           63.74 &    60.36 (3.51) \\
43  &        10 - 8 - 17 &     RAdam &                  4 &           63.67 &    62.49 (1.81) \\
44  &            40 - 20 &       SGD &                  4 &           63.61 &    63.18 (0.49) \\
45  &       30 - 20 - 17 &     RAdam &                  2 &           63.33 &    60.86 (2.45) \\
46  &        10 - 8 - 17 &     AdamW &                  1 &           63.27 &    61.22 (1.77) \\
47  &             10 - 5 &      Adam &                  1 &            63.20 &    61.32 (1.75) \\
48  &         10 - 7 - 4 &     AdamW &                  1 &           63.06 &    61.79 (1.23) \\
49  &         10 - 7 - 4 &     RAdam &                  4 &           62.99 &    61.16 (1.84) \\
50  &         10 - 7 - 4 &     AdamW &                  5 &           62.99 &    60.57 (2.64) \\
51  &        10 - 8 - 17 &     RAdam &                  5 &           62.86 &    61.41 (2.17) \\
52  &        10 - 8 - 17 &      Adam &                  1 &           62.45 &    61.52 (0.86) \\
53  &         10 - 7 - 4 &     RAdam &                  1 &           62.31 &    61.43 (1.10) \\
54  &         10 - 7 - 4 &     RAdam &                  5 &           62.24 &    61.86 (0.56) \\
55  &         10 - 7 - 4 &      Adam &                  4 &           62.18 &    61.32 (0.75) \\
56  &             10 - 5 &     AdamW &                  4 &           62.11 &    61.11 (1.67) \\
57  &       40 - 30 - 20 &     RAdam &                  2 &           62.11 &    60.66 (1.67) \\
58  &        10 - 8 - 17 &      Adam &                  4 &            61.90 &    61.09 (1.36) \\
59  &             10 - 5 &     RAdam &                  4 &            61.70 &    60.39 (1.58) \\
60  &            40 - 20 &     RAdam &                  3 &           61.43 &    58.48 (2.73) \\
61  &        10 - 8 - 17 &     AdamW &                  4 &           61.29 &    60.84 (0.40) \\
62  &             10 - 5 &     RAdam &                  1 &           61.16 &    60.61 (0.48) \\
63  &             10 - 5 &      Adam &                  4 &           61.16 &    59.25 (1.65) \\
64  &         10 - 7 - 4 &      Adam &                  5 &           61.02 &    59.57 (1.66) \\
65  &        10 - 8 - 17 &     AdamW &                  5 &           60.95 &    60.72 (0.20) \\
66  &         10 - 7 - 4 &     AdamW &                  4 &           60.82 &    60.68 (0.18) \\
67  &             10 - 5 &     AdamW &                  1 &           60.68 &    60.02 (0.91) \\
68  &        10 - 8 - 17 &      Adam &                  5 &           60.54 &    59.68 (1.06) \\
69  &             10 - 5 &      Adam &                  5 &           60.27 &    58.59 (1.78) \\
70  &             10 - 5 &     AdamW &                  5 &           60.14 &    58.75 (1.21) \\
71  &         10 - 7 - 4 &       SGD &                  5 &            60.00 &    54.97 (5.21) \\
72  &             10 - 5 &     RAdam &                  5 &            60.00 &    58.59 (1.36) \\
73  &            40 - 20 &      Adam &                  2 &           59.93 &    56.94 (3.91) \\
74  &        10 - 8 - 17 &      Adam &                  6 &           59.52 &   48.80 (13.72) \\
75  &        10 - 8 - 17 &       SGD &                  1 &           59.39 &    57.19 (2.15) \\
76  &        10 - 8 - 17 &     RAdam &                  6 &           58.91 &    57.35 (1.37) \\
77  &            40 - 20 &     AdamW &                  2 &           58.84 &    58.23 (0.69) \\
78  &             10 - 5 &     RAdam &                  6 &           58.78 &    57.60 (1.49) \\
79  &       40 - 30 - 20 &       SGD &                  6 &           58.16 &    56.12 (1.87) \\
80  &        10 - 8 - 17 &       SGD &                  5 &           57.82 &    56.28 (2.32) \\
81  &        10 - 8 - 17 &     RAdam &                  2 &           57.76 &    54.86 (2.52) \\
82  &             10 - 5 &       SGD &                  5 &           57.55 &    55.53 (2.46) \\
83  &       40 - 30 - 20 &     AdamW &                  2 &           57.55 &    53.27 (4.62) \\
84  &             10 - 5 &      Adam &                  6 &           57.41 &    57.09 (0.34) \\
85  &         10 - 7 - 4 &       SGD &                  1 &           57.28 &    55.62 (1.57) \\
86  &        10 - 8 - 17 &       SGD &                  4 &           57.21 &    56.76 (0.73) \\
87  &        10 - 8 - 17 &     AdamW &                  6 &            56.80 &    56.35 (0.52) \\
88  &       30 - 20 - 17 &     RAdam &                  3 &           56.46 &    53.45 (2.90) \\
89  &         10 - 7 - 4 &      Adam &                  6 &           56.46 &   48.39 (13.05) \\
90  &             10 - 5 &     AdamW &                  6 &           56.39 &    53.63 (3.89) \\
91  &         10 - 7 - 4 &       SGD &                  4 &           56.33 &    55.08 (1.17) \\
92  &       30 - 20 - 17 &       SGD &                  6 &           56.12 &    54.72 (1.43) \\
93  &             10 - 5 &       SGD &                  1 &           55.92 &    55.01 (1.23) \\
94  &         10 - 7 - 4 &     RAdam &                  6 &           55.85 &    54.15 (1.74) \\
95  &             10 - 5 &       SGD &                  4 &           55.78 &    54.40 (1.26) \\
96  &       40 - 30 - 20 &     RAdam &                  5 &           55.78 &    53.76 (2.71) \\
97  &         10 - 7 - 4 &     AdamW &                  6 &           55.37 &    55.17 (0.20) \\
98  &             10 - 5 &     RAdam &                  2 &           54.97 &    54.47 (0.48) \\
99  &         10 - 7 - 4 &     RAdam &                  2 &           54.97 &    52.63 (2.46) \\
100 &        10 - 8 - 17 &      Adam &                  2 &            54.90 &    51.36 (3.16) \\
101 &        10 - 8 - 17 &     AdamW &                  2 &           54.63 &   45.42 (10.94) \\
102 &       40 - 30 - 20 &      Adam &                  2 &           54.35 &   45.67 (10.98) \\
103 &             10 - 5 &     AdamW &                  2 &           54.22 &    52.04 (2.25) \\
104 &            40 - 20 &      Adam &                  3 &           54.15 &   46.98 (11.83) \\
105 &       40 - 30 - 20 &     RAdam &                  3 &           53.81 &    53.06 (0.79) \\
106 &            40 - 20 &     AdamW &                  3 &           53.67 &    51.00 (2.59) \\
107 &             10 - 5 &      Adam &                  2 &           53.67 &    51.99 (1.74) \\
108 &       30 - 20 - 17 &      Adam &                  2 &           52.72 &    44.19 (9.90) \\
109 &            40 - 20 &       SGD &                  6 &           52.38 &    51.59 (1.15) \\
110 &             10 - 5 &     RAdam &                  3 &           52.31 &    49.32 (4.28) \\
111 &         10 - 7 - 4 &     RAdam &                  3 &           52.24 &    46.37 (5.18) \\
112 &         10 - 7 - 4 &       SGD &                  6 &            51.90 &    48.16 (3.43) \\
113 &         10 - 7 - 4 &      Adam &                  2 &           51.63 &    44.44 (9.76) \\
114 &         10 - 7 - 4 &     AdamW &                  2 &            51.50 &   39.39 (10.49) \\
115 &             10 - 5 &      Adam &                  3 &           51.29 &    46.46 (4.53) \\
116 &        10 - 8 - 17 &       SGD &                  6 &           51.09 &    49.89 (1.11) \\
117 &             10 - 5 &       SGD &                  6 &           50.68 &    50.30 (0.45) \\
118 &        10 - 8 - 17 &     RAdam &                  3 &           50.48 &    50.02 (0.45) \\
119 &       30 - 20 - 17 &     AdamW &                  2 &           50.41 &     50.41 (nan) \\
120 &         10 - 7 - 4 &     AdamW &                  3 &           50.07 &    41.56 (8.37) \\
121 &        10 - 8 - 17 &      Adam &                  3 &           49.46 &    41.18 (8.07) \\
122 &       30 - 20 - 17 &      Adam &                  3 &           49.12 &    46.96 (3.33) \\
123 &             10 - 5 &     AdamW &                  3 &           48.64 &    42.63 (8.17) \\
124 &         10 - 7 - 4 &      Adam &                  3 &           48.64 &    38.43 (8.84) \\
125 &       40 - 30 - 20 &       SGD &                  2 &            48.10 &    45.97 (1.97) \\
126 &       40 - 30 - 20 &       SGD &                  3 &           47.96 &    46.26 (2.44) \\
127 &            40 - 20 &       SGD &                  3 &           46.67 &    44.06 (2.33) \\
128 &       30 - 20 - 17 &       SGD &                  2 &           46.53 &    45.37 (1.72) \\
129 &            40 - 20 &       SGD &                  2 &           46.19 &    44.97 (1.89) \\
130 &            40 - 20 &     RAdam &                  7 &           46.05 &    45.19 (0.79) \\
131 &             10 - 5 &     RAdam &                  7 &           45.99 &    41.20 (5.75) \\
132 &            40 - 20 &     AdamW &                  7 &           45.78 &    44.03 (1.74) \\
133 &       30 - 20 - 17 &       SGD &                  3 &           45.58 &    42.70 (2.96) \\
134 &       30 - 20 - 17 &     RAdam &                  7 &           45.44 &    42.88 (2.48) \\
135 &       40 - 30 - 20 &     AdamW &                  3 &            45.10 &    37.25 (6.80) \\
136 &       40 - 30 - 20 &     RAdam &                  7 &           44.76 &    43.58 (1.12) \\
137 &       40 - 30 - 20 &      Adam &                  3 &           44.69 &    40.88 (6.54) \\
138 &            40 - 20 &      Adam &                  7 &           44.56 &    37.07 (6.48) \\
139 &             10 - 5 &     AdamW &                  7 &           44.56 &    40.18 (6.01) \\
140 &       40 - 30 - 20 &      Adam &                  7 &           43.54 &    39.82 (5.64) \\
141 &        10 - 8 - 17 &       SGD &                  2 &           43.13 &    41.91 (1.62) \\
142 &       40 - 30 - 20 &     AdamW &                  7 &           43.06 &    38.55 (4.90) \\
143 &             10 - 5 &      Adam &                  7 &           42.99 &    39.32 (5.23) \\
144 &        10 - 8 - 17 &     RAdam &                  7 &           42.99 &    40.29 (2.42) \\
145 &         10 - 7 - 4 &     AdamW &                  7 &           42.59 &    36.42 (5.35) \\
146 &        10 - 8 - 17 &       SGD &                  3 &           42.38 &    39.77 (2.44) \\
147 &       30 - 20 - 17 &      Adam &                  7 &           42.31 &    38.89 (4.86) \\
148 &         10 - 7 - 4 &       SGD &                  2 &           42.18 &    39.80 (3.03) \\
149 &        10 - 8 - 17 &      Adam &                  7 &           42.04 &    38.77 (4.75) \\
150 &        10 - 8 - 17 &     AdamW &                  7 &            41.70 &    36.12 (4.83) \\
151 &         10 - 7 - 4 &       SGD &                  3 &           41.16 &    39.50 (2.31) \\
152 &         10 - 7 - 4 &     RAdam &                  7 &           40.34 &    35.67 (4.05) \\
153 &             10 - 5 &       SGD &                  2 &           39.39 &    38.71 (0.63) \\
154 &             10 - 5 &       SGD &                  3 &           38.03 &    36.42 (2.02) \\
155 &            40 - 20 &       SGD &                  7 &           37.28 &    37.01 (0.31) \\
156 &        10 - 8 - 17 &       SGD &                  7 &           36.39 &    34.99 (2.26) \\
157 &       40 - 30 - 20 &       SGD &                  7 &           36.19 &    34.92 (1.29) \\
158 &         10 - 7 - 4 &       SGD &                  7 &           35.51 &    34.33 (1.10) \\
159 &       30 - 20 - 17 &       SGD &                  7 &           35.37 &    34.44 (0.99) \\
160 &        10 - 8 - 17 &     AdamW &                  3 &           35.03 &    33.90 (0.98) \\
161 &             10 - 5 &       SGD &                  7 &           33.95 &    33.63 (0.31) \\
\midrule
162 &         10 - 7 - 4 &      Adam &                  7 &           33.33 &    33.33 (0.00) \\
\end{longtable}
\end{small}
\end{center}




% -------------- Extensive conclusion from thesis -------------


% A novel logic learning pipeline has been introduced that makes use of trained real-valued neural networks, to derive logic in three different ways: as a direct translation to arithmetic circuits and by using quantized activations of the net to train random forests and LogicNets, which can be translated separately into logic circuits. Lastly, an additional option has been provided that trains random forests directly on the data before turning them into logic. For all methods, a number of hyper-parameters has been suggested. \\

% The proposed logic derivation pipeline was evaluated on two biomedical data sets (GIB and VACS). For each of those, one rather big and one rather small real-valued neural network was used as input to the logic derivation pipeline, using only those that performed the best on the test data. To each of them, multiple quantization schemes were applied, in order to find the best possible arithmetic circuit baseline models. Two quantization schemes were selected individually for each case: one with a high number of total bits and one with a low number of total bits. Those were used for experiments with LogicNets and random forests as intermediate steps of the logic derivation pipeline, but also for training random forests directly on the data and translating them into logic independently. \\

% To summarize, the proposed methods show clear improvements in both the capability of generalization with logic and a decreased logic complexity, driving implementability and interpretability. Within that, the logic benefits from using small neural networks and simple feed-forward architectures. Using small architectures also has the advantage of saving computational resources and computing time. As a side-observation, it can be noted that searching for a real-valued neural network that perfectly fits the data, in order to use it as a starting point of the pipeline is not worth the effort. Instead it should be searched for rather small architectures and the main computational resources should instead go into testing different logic configurations, as no clear pattern was found which hyper-parameters perform better than others. However, for the search of a real-valued neural network configuration, it was observed that the SGD optimizer performed worse on the GIB and VACS data than others, while no clear benefit was observed of using one specific data normalization technique. \\

% The pipeline generally shows good results for small quantization schemes, while for large quantization schemes there is room for improvement or other available methods should be preferred. Especially, the usage of random forests, either trained directly on the data or on neural network activations performs well, while using LogicNet on neural network activations does not show any capability of generalization. This can also be due to bitwise training methods in general not performing as well as none-bitwise training methods. A recommendation of the usage of the derived methods can be summarized as follows:  

% \begin{itemize}
% \item It should be started with small real-valued neural networks and small quantization schemes, to derive an arithmetic circuit.
% \item When the arithmetic circuit performs poorly, the logic learning pipeline helps to increase the chance of finding a well-generalizing logic circuit that is smaller in terms of size and complexity and better in terms of accuracy. 
% \item When the arithmetic circuit already performs well, thus forms a strong baseline, the logic learning pipeline can help finding a less bloated logic that achieves similar results. 
% \item The logic pipeline can in general help to bring light to neural networks as black-boxes by deriving interpretable reports and finding dependencies on inputs.
% \end{itemize}


